The good, the bad and the ugly sides of data augmentation: An implicit spectral regularization perspective

Data augmentation (DA) is a powerful workhorse for bolstering performance in modern machine learning. Specific augmentations like translations and scaling in computer vision are traditionally believed to improve generalization by generating new (artificial) data from the same distribution. However, this traditional viewpoint does not explain the success of prevalent augmentations in modern machine learning (e.g. randomized masking, cutout, mixup), that greatly alter the training data distribution. In this work, we develop a new theoretical framework to characterize the impact of a general class of DA on underparameterized and overparameterized linear model generalization. Our framework reveals that DA induces implicit spectral regularization through a combination of two distinct effects: a) manipulating the relative proportion of eigenvalues of the data covariance matrix in a training-data-dependent manner, and b) uniformly boosting the entire spectrum of the data covariance matrix through ridge regression. These effects, when applied to popular augmentations, give rise to a wide variety of phenomena, including discrepancies in generalization between over-parameterized and under-parameterized regimes and differences between regression and classification tasks. Our framework highlights the nuanced and sometimes surprising impacts of DA on generalization, and serves as a testbed for novel augmentation design.

==> files/abstract_old.tex <==
Data augmentation (DA) is often critical to the success of modern machine learning, yet the use of DA is usually based upon trial-and-error and a precise and interpretable characterization of the impact of different augmentations on generalization is largely missing. 
A more grounded theoretical foundation is needed to understand and characterize the impact of different augmentations and serve as an interpretable testbed to guide practice moving forward. 

In this work, we develop a new theoretical framework for understanding the impact of DA on generalization from a spectral perspective. Specifically, we analyze augmented empirical risk minimization (aERM) under any augmentation that is \emph{unbiased} and is applied independently to training examples on-the-fly. By leveraging finite analysis techniques in the benign overfitting literature, we derive matching non-asymptotic upper and lower bounds on the generalization error for both regression and classification. 
Our theory provides higher resolution on how DA impacts the generalization with respect to the bias and variance and reveals that DA creates effects of ridge regularization along with data distribution manipulation through implicit data-dependent regularization. 
We also discover an intriguing disparity between DA in over-and under-parametrized regimes, where we found group invariance is not always beneficial in the former scenario. 

Our framework also serves as a testbed for novel augmentations.
In particular we propose a new ``randomized rotation" augmentation derived from the equivalence of random rotation in high dimensional space that has excellent generalization performance on par with optimal ridge regression while remaining far more stable across its hyperparameters. Finally, we conduct empirical experiments to validate our observations. (\henry{more persuasive arguments hv to be added regarding experiments, btw, the abstract is too long atm right??})

==> files/addn_experiments.tex <==
\section{Additional Experiments}\label{more_exp}

In Fig. \ref{mask_in_re}, we illustrate the impact of input spectrum on the random mask augmentation complementing the experiments in Section 5.2.

\begin{figure}[htbp!]
    \centering
    \setcounter{subfigure}{0}
      {\includegraphics[width=1\textwidth]
   {imgs/inorder_reverse_mask.png}\vspace{-0mm}}
    \caption{\footnotesize{\textbf{Impact of covariance spectrum on the random mask augmentation in $p=128$ dimensions.} We consider three different augmentations strategies in a decaying spectrum where across features, augmentation intensities re uniform (left),  increasing with feature variance (middle}, and decreasing with feature variance (right). A negative relation between augmentation and data covariance is better for bias and worse for the variance, while the former strategy is generally better for a wider range of augmentation in the overall MSE.\label{mask_in_re}}
\end{figure}

==> files/background.tex <==
\section{Background and Related Work}


%\subsection{Preliminaries}
%Setup and notations? 
We organize our discussion of related work into two verticals: a) historical and recent perspectives on the role of data augmentation, and b) recent analyses of minimum-norm and ridge estimators in the overparameterized regime.

\vspace{-3mm}
\subsection{Data augmentation} 

Recent work in building a theoretical foundation for DA has already provided insights into the invariance properties induced by structured group-level (rotation, translation) augmentations~\cite{chen2020group} and the effect of single virtual samples on generalization~\cite{wu2020generalization}. The authors in~\cite{chen2020group} propose a framework based on the group theory and explain that the symmetrization help model generalize by variance reduction. However, our work discovers that in overparametrized regime the whole story about DA is more than just the transformation invariance but involves the data spectrum, where we show that group invariant alone could even be harmful by making the data spectrum symmetry. A close work related to us~\cite{wu2020generalization} also studies the linear model generalization with DA in overparametrized regime, but they consider pre-comput based augmentation method and the augmentation class they consider, e.g. label invariant, is hardly held in practice. They explain that DA has the ability of enlarging the span of training data and enhance the explicit regularization. However, there work is applicable only to regularized estimator, hence the alone effect from DA entangles with explicit regularization. Furthermore, the key spectrum aspect of generalization in the regime is missing.~\cite{dao2019kernel} proposes a Markov process based framework to model the DA, and builds up close relation between DA and kernel classifier, which is generated from the augmented data distribution. While they have analyzed a similar objective of augmentation population based objective like us but with more involved data augmentation modeling, the gap between how DA affects augmented distribution and then affect on the final generalization still exists. Very recently,~\cite{shen2022data}’s work investigate the DA from a dynamic perspective, and find that the feature manipulation effect of DA during the learning processing, where relatively important features are easier to learn with DA. However, their augmentation is very specific which loses the generality to study how different augmentations impact the generalization.


%in modern ML.}
Data augmentation is a common technique used to enhance model generalization. In general, when augmenting data, we transform the original data  $(\x, y)$ by applying a mapping $g(\x, y)$. The transformation can be broadly classified as either label-invariant or label-variant \cite{wu2020generalization}. In the former, the transformation does not alter the label, i.e., $g(\x,y)=g(\x)$, while it may change both the covariate and the label in the latter. The former class includes adding Gaussian noise, random mask, and random rotation, while the later subsumes mixup \cite{zhang2017mixup}.
We focus on the former class in this work.

Early statistical theory of DA showed that adding random noise to data points is equivalent to Tikhonov regularization~\cite{bishop1995training} and vicinal risk minimization~\cite{chapelle2001vicinal,zhang2017mixup}.  The intuition is that by adding isotropic Gaussian noise to data samples, we expand the data manifold uniformly with respect to its features. This also creates the question of whether other manifold expansion strategies could lead to better performance, and conversely, what is the data augmentation that leads to the optimal performance? Another set of recent works explores the common intuition that data augmentation helps insert beneficial group-invariances into the learning process \cite{cohen2016group, raj2017local, mroueh2015learning, bruna2013invariant}. These works generally consider cases in which the group structure is explicitly present in the model design via convolutional architectures \cite{cohen2016group, bruna2013invariant} or feature maps approximating group-invariant kernels \cite{raj2017local, mroueh2015learning}. While we do not specifically adopt this invariance perspective, we instead focus on the implicit \textit{spectral} effects induced by DA, with an emphasis on generalization error in overparameterized settings.
%\vidya{There is one set of citations missing here on DA and invariances. See our proposal draft for a list of citations --- we should add one sentence on this}\chiraag{added}

Several recent works have focused on
understanding the effect of data augmentation on model generalization. 
The empirical studies of \cite{gontijo2020affinity} have highlighted the importance of both affinity and diversity in augmentations. They argue that in many cases the need for diverse new examples drives the use of augmentation methods that introduce samples that are out-of-distribution (OOD), in the sense that they don't resemble other samples observed in the data.
In theoretical works, a group-theoretic framework for DA was put forward by \cite{chen2020group}, and DA was shown to induce helpful explicit regularization and reduce the variance of the maximum-likelihood-estimator~\cite{chen2020group}. They provide some initial results in the underparameterized regime for the aERM formulation that we study in this work. However, their results either apply in underparameterized settings or depend on additional \textit{explicit} regularization, which can entangle with the \textit{implicit} regularization effect from data augmentations. 
Additionally, by considering stochastic off-manifold (or out of group) transformations (as discussed in \cite{gontijo2020affinity}), we show that more explicit bounds can be derived that depend on the spectral properties of our data and the applied augmentation.

Another recent effort \cite{wu2020generalization} characterizes the impact of augmentations on the generalization error for linear regression and considers the improvement in risk when a single augmented sample (or a finite number of such samples) is added to the training set. We empirically consider the effects of this ``pre-computed'' mode of DA, but our primarily analysis operates in a different setting which more closely models the effect of ``on-the-fly'' augmentations applied during training. Moreover, the label-invariant transformations $g$ considered in \cite{wu2020generalization}  must be linear and the transformed data $g(\x)$ must satisfy $g(\x)^\top \theta^* = x^\top \theta^*$, which is a stricter condition than we impose on the augmentation class. 

% However, they does not the analyze the augmentation from a statistical perspective and does not
% make the connection between the spectral properties of data and augmentation. 
\henry{talk about what hvnt been done in more details\cite{chen2020group}\cite{wu2020generalization}} \vidya{Concrete suggestions:~\cite{chen2020group} operates in underparameterized regime (or overparameterization but with explicit regularization) and makes an in-distribution assumption on DA which is highly restrictive. Many of the interesting DAs we study induce an OOD effect (point to examples and connect to perspective in [8]). More mathematically precise comparison is needed for~\cite{wu2020generalization}. What does ``single augmented sample" mean? And if they are studying generalization why is it not a statistical perspective?}
\vidya{Suriya paper also needs to be added and discussed (as very recent work so the comparison can be relatively high level). In particular they have a feature learning/manipulation perspective that is worth highlighting.}\henry{ok! i am gonna read \cite{wu2020generalization} in details and also Suriya's paper}

\subsection{Interpolation of noise in overparameterized settings}
Our work leverages recent results in linear regression in \textit{overparameterized} settings. Following the definition of \cite{dar2021farewell}, we characterize such works by their explicit focus on models which achieve close to zero training loss and which have high complexity (taking into account any regularization in the learning procedure) relative to the number of training samples.
\vidya{Define overparameterization formally here: our survey paper will be helpful as we provide a formal definition.}
Specifically, many of these works provide finite-sample analysis for the risk of the least-squared estimator (LSE) and ridge estimators \cite{bartlett2020benign, tsigler2020benign}. This line of research finds that the 
mean squared error (MSE) comprising of
the bias and variance can be characterized in terms of effective ranks of the data covariance $\SIG:=\E\x\x^\top$. In particular, in the overparameterized setting, they show that, contrary to traditional wisdom, overfitting (perfect interpolation of the data) may not have a harmful effect on the generalization error. These types of analyses have also been applied to the classification setting, where a similar type of ``benign overfitting'' is also shown to occur \cite{muthukumar2020class, cao2021risk, wang2021binary, chatterji2021finite}. Our work adopts the general classification setting of \cite{muthukumar2020class}, but allows for a more general non-Gaussian design.

% For example in the LSE \cite{bartlett2020benign}, we have
% \begin{align*}
%     &\mathrm{MSE} \lesssim {\rm Bias} + {\rm Variance},\\
%     &{\rm Bias} \lesssim \|\TBS\|_{\SB}^2 +  \|\TAS\|_{\SA^{-1}}^2\lambda_{k+1}^2\rho_k^2,~~ {\rm Variance} \lesssim \frac{k}{n} + \frac{n}{R_k},
% \end{align*}
% where $\lambda_i$ are the eigenvalues of $\SIG$, and $r_k,~R_k$ are the {\em effective ranks} defined by $$\rho_k = \frac{\sum_{i>k}\lambda_i}{n\lambda_{k+1}},~R_k=\frac{(\sum_{i>k}\lambda_i)^2}{\sum_{i>k}\lambda_i^2},$$ and $k$ defines an index partitioning the spectrum into the spiked and residual parts. 

The key discovery in these works is the condition of the rise of benign overfitting. They discover that the data spectrum needs to decay at a balanced pace:
it has to decay fast so that the signal is easier to fit, while not fast enough or the noise gets fit well too. 
While explicit regularization directly prevent a model from overfitting the data by constraining the function complexity, DA has an additional effect of manipulating the data distribution and thus its spectrum based on the training data itself. 
\henry{i think explicit regularization does not change the data spectrum as DA. The effective ranks do change, but it is not equivalent to a change of data distribution as DA does in our equivalence established in eq (8). Hence, i want to argue that DA has two effects: 1. implicit fixed regularization just as fixed explicit regularization that constrained the function norm (or constrainning the model complexity) and  2. change of data distribution based on the data spectrum itself. the point 2 is made precise in (8). it really does like change the data distribution. and if you look at the effective ranks, its like change of eigenvalues and also has a l2 regularization together, on the other hand, the l2 regularization alone can not absorbed to a change of lambda and so its not equivalent to a spectrum change}
As we will show in this work, depending on the type of augmentation, this two can have sum effect to be harmful or helpful in model generalization.
\henry{we havent really shown this yet, but as i wrote it i felt its a good story!}


% 1. the bias is small when the true model parameter has small component in the data eigenspace with smaller eigenvalues, and 2. the variance is small when the small eigenspace has a large number of non-negligible eigenvalues. 

% To resolve this dilemma, a common practice is to use an explicit regularization that increases the eigenvalues in the residual spectrum so that the variance is decreased and the bias remains in the same scale. As we will uncover in this work, DA can have both the effects of changing and regularizing the data spectrum in many different ways, depending on the type of augmentation applied.


% From the expression, we immediately observe the tension between the bias and variance: 1. the bias is small when the optimal parameter has small variance in the eigenspace with smaller eignevalues. 2. the variance is small when the smaller eigenspaces has non-negligible eigenvalues. To solve the dilemma, a common practice is to use an explicit regularization that increases the eigenvalues in residue spectrum so that the variance is decreased ($R_k$ is increased) and the bias remains in the same scale ($\SB$ is unaffected). As we will uncover in this work, DA have both the effect of changing and regularizing the data spectrum in many different ways with various types of augmentation. Hence, in high level sense, the augmentation adapts the spectrum by itself to fight the overfitting problem.

Modern machine learning models operate in the overparameterized regime and have achieved great success.
However, the seeming contradiction to the common wisdom of overfitting has remained a mystery. Recently, several works \cite{hastie2019surprises, bartlett2020benign, tsigler2020benign, belkin2020two, muthukumar2020harmless, wang2021binary} have have made first-step explanations towards understanding the success of deep learning models by offering insights into linear models through modern analysis. Among these works, \cite{bartlett2020benign,tsigler2020benign,muthukumar2020class,zou2021benign} have derived the generalization bounds with non-asymptotic analysis, quantifying the spectral conditions under which the risk is vanishing despite perfect fitting of the noise. In this work, we expand the applicability of these works to the scenario of learning with data augmentation, identify sufficient conditions under which the risk will be vanishing, and compare the generalization performance of different data augmentations.



==> files/class_results_old.tex <==
\subsection{Classification analysis}\label{class-results}
In this subsection, we consider the generalization of DA for classification tasks. We follow a similar path as in regression by introducing the setup and appealing to the connection between the DA and ridge estimator and the deterministic approximation strategy for the analysis. While the results in this section operate under stronger assumptions, we provide a similar set of results to the regression case, with the primary aim of comparing the generalization behavior of DA between regression and classification settings.
%\henry{talk about the limitation on the model assumption}\chiraag{done}

\subsubsection{Preliminaries}
We adopt the signed model from \cite{muthukumar2020class}. However, the analysis can be performed similarly on the Gaussian mixture models in the setting of \cite{wang2021binary}. We defer analysis in the latter setting to a later work.
Specifically, we consider the case where each observation $y_i \in \{-1,1\}$.
Given a target vector $\theta^* \in \reals^d$ and a label noise parameter $0 \leq \nu^* <1/2$, we assume the data are generated according to:
\begin{equation}
y_i=\begin{cases}
          \sgn(\x_i^\top \T^*) \quad &\text{with probability} \, 1-\nu^* \\
          -\sgn(\x_i^\top \T^*) \quad &\text{with probability} \, \nu^* \\
     \end{cases}
\end{equation}
%For ease of analysis, we assume in this section that $\x_i \sim \mathcal{N}(\mathbf{0}, \SIG)$ with diagonal covariance; however, our results also extend to the weaker assumption of sub-gaussian, but independent features. 
To get insights from cleaner analysis, we make a \textit{1-sparse} assumption on the true signal $\T^* = \frac{1}{\sqrt{\lambda_t}} \e_t$; this assumption is without loss of generality since our analysis makes use of a connection to ridge regression, which is agnostic to orthonormal transformations. 
We denote $\x_{\text{sig}}:=\x_t$ to emphasize the signal feature.
Motivated by recent results which demonstrate the effectiveness of training with the squared loss for classification tasks, we study the classification risk of the estimator $\Th$ which is computed by solving the aERM objective \ref{DAobj} on the binary labels $y_i$. 

%Our analysis of the classification risk draws from Proposition 17 of \cite{muthukumar2020class}, which, under the above signal model, expresses the excess risk of a given estimator as 
In \cite{muthukumar2020class}, the authors showed that two quantities, \textit{survival} and \textit{contamination}, play key roles in characterizing the risk, akin to the bias and variance in the regression task. Their definitions are given below:
\begin{definition}\label{su_cn_def}
Given an estimator $\hat{\theta}$, its survival (SU) and contamination (CN) are defined as 
\begin{align}
    \mathrm{SU(\Th)} = \sqrt{\lambda_t}\Th_t,~~\mathrm{CN(\Th)} =  \sqrt{\sum_{j=1, j\neq t}^p \lambda_j \Th_j^2}.
\end{align}
\end{definition}
When the input feature has independent Gaussian features, the authors in \cite{muthukumar2020class} derived the POE in a closed-form as
\begin{equation}\label{class-risk}
    \text{POE}(\Th) = \frac{1}{2} - \frac{1}{\pi}\tan^{-1}\frac{\mathrm{SU(\Th)}}{\mathrm{CN(\Th)}}.
\end{equation}
The generalization error depends on the ratio between SU and CN, reminiscent of system performance depending on the signal-to-noise ratio (SNR) in signal processing. In this work, we prove that a similar principle arises when we consider training with data augmentation in more general correlated input distributions.

Formally, we make the following assumption on the input distribution for our classification analysis:

\begin{assumption}
    The input can be factored as $\x=\SIG^{\frac{1}{2}} \z$, where $\SIG \succeq 0$ is diagonal, and $\z$ is a sub-gaussian random vector with norm $\sigma_x$ comprising of two parts: the signal feature $\z_t$ and the noise part $[\z_1,\dots,\z_{t-1},\z_{t+1},\dots,\z_p]$. We denote $\x_{\text{sig}}=\x_t$ and $\x_{\text{noise}}=[\x_1,\dots,\x_{t-1},\x_{t+1},\dots,\x_p]^T$. We assume the signal and noise are independent, i.e., $\x_{\text{sig}}\perp  \x_{\text{noise}}$.
\end{assumption}

% The signal feature $\x_{\text{sig}}:=\x_1$ is independent of the noise features $\x_{\text{noise}}:=[\x_2,\x_3,\dots,\x_p]$ and both of them are sub-Gaussian with norm $\sigma_x$.

% \begin{remark}
% Not only does assumption 2 subsume the Gaussian class, but it also covers the uniform distribution on sphere, and sub-Gaussian with independent components. 
% \end{remark}

\paragraph{Analysis approach.}
Similar to the regression case, the analysis consists of 1) expressing the excess risk in terms of $\BT$, the estimator corresponding to the averaged augmented covariance $\mathbb{E}_{\x}[\text{Cov}_g(\x)]$, 2) arguing that the survival and contamination can be viewed as the equivalent quantities for a ridge estimator with a modified data spectrum, and 3) upper and lower bounding the survival and contamination of this ridge estimator.

\subsubsection{Classification analysis for unbiased augmentations}
Now we present our main theorem on the generalization bound for classification task. The detailed proof is deferred to Appendix \ref{main_proof_cls}.

\begin{theorem}[\textbf{Bounds on Probability of Classification Error}]\label{thm2} 
    Consider the classification task under the model and assumption described in Section \ref{class-results} where the true signal $\theta^*$ is 1-sparse. Let $\HT$ be the estimator solving the aERM objective in (\ref{DAobj}). Denote $\boldsymbol{\Delta}_G := \|\text{Cov}_G(\X)-\mathbb{E}_{\x}[\text{Cov}_g(\x)]\|$, let $t \leq n$ be the index (arranged according to the eigenvalues of ${\SIG}_{\text{aug}}$) of the non-zero coordinate of the true signal, $\tilde{\SIG}_{\text{aug}}$ be the leave-one-out modified spectrum corresponding to index $t$, $\kappa$ the condition number of $\SIG\mathbb{E}_{\x}[\mathrm{Cov}_g(\x)]^{-1}$, and $\tilde{\X}_{\text{aug}}$ be the leave-one-column-out data matrix corresponding to column $t$. 
    
    Suppose data augmentation is performed independently for $\x_{sig}$ and $\x_{noise}$, and there exists a $t \leq k \leq n$ such that with probability at least $1-\delta$, the condition numbers of $n \I + \tilde{\X}^{\text{aug}}_{k+1:p}(\X^{\text{aug}}_{k+1:p})^\top$ and 
    $n \I + {\X}^{\text{aug}}_{k+1:p}(\X^{\text{aug}}_{k+1:p})^\top$
    are at most $L$, $\boldsymbol{\Delta}_G < c$ for some $c<1$, and that of $n\I + \X\X^\top$ is at most $L_1$. Then as long as $\Vert \BT - \HT\Vert_{\SIG} = O(SU)$ and $\Vert \BT - \HT\Vert_{\SIG} = O(CN)$, for any $\delta'>0$, with probability $1-\delta-\exp(-\sqrt{n})-5n^{-1}$, we have an upper bound of Probability of classification error (POE) consisting of the {\color{blue}survival} (SU), {\color{red}contamination} (CN), and  {\color{olive}error multiplier} (EM):
    \begin{align}\label{thm2_poe}
        \mathrm{POE}(\HT)\leq \mathbb{P}(\x_{\text{sig}}^2 < \delta') + 3\exp\left(-\frac{\delta'}{\lambda_1\sigma_x^2}\frac{{\color{blue}\mathrm{SU}}^2}{{\color{olive}\mathrm{EM}}^2{\color{red}\mathrm{CN}}^2}\right),
    \end{align}
    where
    \begin{align}
        \frac{\lambda^{\text{aug}}_t(1-2\nu^*)\left(1-\frac{k}{n}\right)}{L\left(\lambda^{\text{aug}}_{k+1}\rho_k(\SIG_{\text{aug}};n) + \lambda_t^{\text{aug}}L\right)}~\lesssim~\underbrace{{\color{blue}\mathrm{SU}}}_{\text{Survival}}&~\lesssim~\frac{L\lambda^{\text{aug}}_t(1-2\nu^*)}{\lambda^{\text{aug}}_{k+1}\rho_k(\SIG_{\text{aug}};n) + L^{-1}\lambda^{\text{aug}}_t\left(1-\frac{k}{n}\right)},\\
        \sqrt{\frac{\tilde{\lambda}^{\text{aug}}_{k+1}\rho_{k}(\tilde{\SIG}_{\text{aug}}^2;0)}{LL_1^2\lambda_1^2\rho^2_0(\SIG_{\text{aug}};n)}}~\lesssim~
        \underbrace{{\color{red}\mathrm{CN}}}_{\text{Contamination}} &~\lesssim~ \sqrt{(1+\mathrm{SU}^2)L^2\left(\frac{k}{n} + \frac{n}{R_k(\tilde{\SIG}_{\text{aug}};n)}\right)\log n}\\
        0 ~\leq ~\log(\underbrace{{\color{olive}\mathrm{EM}}}_{\text{Error multiplier}})&~\lesssim~ {\kappa^{\frac{1}{2}} \Vert \boldsymbol{\Delta}_G  \Vert }\max\left(\frac{\mathrm{SU}}{\mathrm{CN}}, \frac{\mathrm{CN}}{\mathrm{SU}}\right)
    \end{align}
    Furthermore, if $\x$ is Gaussian and the augmentation modified spectrum $\SIG_{\text{aug}}$ is diagonal then
    \begin{align}
         \mathrm{POE}(\HT) \leq \frac{1}{2} - \frac{1}{\pi}\tan^{-1}\frac{1}{{\color{olive}\mathrm{EM}}}\frac{{\color{blue}\mathrm{SU}}}{ {\color{red}\mathrm{CN}}}\leq {\color{olive}\mathrm{EM}}{\frac{{\color{red}\mathrm{CN}}}{{\color{blue} \mathrm{SU}}}}.
    \end{align}
    

\end{theorem}


\begin{remark}
Based on the expression for the classification error for Gaussian data, we see that, when $\log(EM)$ is small, the condition that the survival is asymptotically greater than the contamination is clearly necessary for the risk to not approach $1/2$ in the limit. We note that in the Gaussian case, matching lower bounds can also be obtained by using the bounds on SU and CN provided above, indicating that the conditions of Theorem \ref{thm2} are actually necessary to obtain good classification performance. In the following corollaries, we demonstrate that this condition may or may not be satisfied, depending on the type of augmentation applied and the original spectrum of the data.
\end{remark}

Considering the expression in \ref{thm2_poe}, we note that the first term can be chosen to be arbitrarily small and the second term is small when the ratio SU/CN is large. Based on the upper and lower bounds provided, we see that these quantities depend crucially on the spectral properties of the induced covariance matrix $\SIG_{aug}$. For favorable classification performance, Theorem \ref{thm2} also requires $t \leq n$. This is a necessary product of our analogy to a ridge estimator and is equivalent to requiring that $\theta_{\text{aug}}^*$ lies within the dominant eigenspace corresponding to the spectrum $\SIG_{aug}$ (a natural requirement for harmless interpolation in ridge regression). Similar to the regresion analysis, our theorem can apply to the Gaussian noise injection augmentation, which, as discussed previously, is equivalent to a ridge regression estimator. These results generalize the bounds in \cite{muthukumar2020class} beyond the ridgeless case (and can yield consistency, e.g. under the bi-level spectrum they consider) and the gaussianaity assumption. For space consideration, we defer the results to Appendix \ref{pf_cls_cor}.

We next consider two different types of augmentation for which the induced covariance $\SIG_{\text{aug}}$ is isotropic, yielding poor generalization in overparameterized settings. The authors in \cite{chen2020group} have argued that group invariance is an important reason of how DA help generalization. However, as we find in the next corollary, the story is very different between over- and under-parametrized regimes. At a high level, we can demonstrate that group invariance has the equivalent effect of ``isotropizing'' the data spectrum, which is undesirable property in overparametrized settings. The formal description is summarized below.


\begin{corollary}
[\textbf{Group invariance does not generalize in overparametrized regime}]\label{gv}
An  augmentation class $\mathcal{G}$ is said to be group invariant if $g(\x)\overset{d}{=} \x,~ \forall g \in \mathcal{G}$. For any such augmentation class, the generalization bound for classification is,
\begin{align}
    \mathrm{SU} &\asymp (1-2\nu) \frac{n}{2n + {p}},\\
        \sqrt{\frac{np}{(n+p)^2}}\lesssim\mathrm{CN} &\lesssim \sqrt{(1+\mathrm{SU}^2)  \frac{np\log{n}}{(n + p)^2}}.
\end{align}
\end{corollary}
\begin{remark}
From the above corollary, it's clear that for underparametrized regime $p\leq n$, SU=$\Theta(1)$, CN=$O(\sqrt{\frac{p\log n}{n}})$ while for overparametrized regime $p\geq n$, SU=$\Theta({\frac{n}{p}})$, CN=$\Omega(\sqrt{\frac{n}{p}})$. Hence, there is a sharp transition of SU to CN ratio between the two regimes. As the ratio is asymptotically zero in the latter, we find that group invariance augmentation can be harmful for generalization in overparametrized regime. 
\end{remark}

The corollary below provides bounds on the survival and contamination for the uniform random mask augmentation.
\begin{corollary}[\textbf{Classification bounds for random mask augmentation}]\label{rm-class}
Let $\HT$ be the estimator computed by solving the aERM objective on binary labels with the  mask probability $\beta$, denote $\psi := \frac{\beta}{1-\beta}$. Then, with probability at least $1-\delta - \exp(-\sqrt{n}) - 5n^{-1}$:
\begin{align}
    \mathrm{SU} &\asymp (1-2\nu) \frac{n}{n\psi + n + {p}},\\
    \mathrm{CN} &\lesssim \sqrt{(1+\mathrm{SU}^2)  \frac{np\log{n}}{(n\psi + p)^2}}\\
    \log(\mathrm{EM}) &\lesssim \frac{\sigma_z^2\log n}{n}\frac{\mathrm{CN}}{\mathrm{SU}}.
\end{align}
Furthermore, the conditions $\Vert \BT - \HT\Vert_{\SIG} = O(SU)$ and $\Vert \BT - \HT\Vert_{\SIG} = O(CN)$ hold for $p \ll n^3$. 
\end{corollary}
As in the group invariance case, we note that when $p$ grows faster than $n$, the survival to contamination ratio is decreasing in $n$, so, even when $EM$ is small, the classification risk cannot be consistent. Indeed, since $\SIG_{aug}$ in this case is isotropic, this behavior is again intimately related to the well-known poor signal recovery in isotropic overparameterized settings.
% \begin{remark}
% It is readily verified that the conditions of Theorem \ref{thm2} are not satisfied if $p$ grows polynomially in $n$ (and the risk is asymptotically $1/2$, by the matching lower bounds in the Appendix). If $p$ and $n$ grow proportionally, then the risk is asymptotically bounded below $1/2$. 
% \end{remark}

To understand which types of augmentations might yield favorable bounds, we consider, as in Corollary \ref{het_mask}, the case of a non-uniform random masking augmentation in which the signal feature is masked with a lower probability the the remaining features (similar results can also be recovered by setting $s < n$ coordinates to have one dropout parameter and the remaining $p-s$ features to have another parameter).

\begin{corollary}[\textbf{Non-uniform random mask}]\label{hrm-class}
Consider the case where the dropout parameter $\psi_j = \frac{\beta_j}{1-\beta_j}$ is applied to the $j$-th feature. For simplicity, we consider the bi-level case where $\psi_j = \psi$ for $j \neq t$. Then, with probability at least $1-\delta - \exp(-\sqrt{n}) - 5n^{-1}$,
\begin{align}
    \mathrm{SU} &\asymp  \frac{1}{\psi_1 + \frac{p\psi_t}{n\psi} + 1}\\
    \mathrm{CN} &\lesssim \sqrt{(1+\mathrm{SU}^2) \frac{np\log{n}}{(n\psi + p)^2}}\\
    \log(\mathrm{EM}) &\lesssim \sqrt{\frac{\psi}{\psi_t}}\frac{\sigma_z^2\log n}{n}\frac{\mathrm{SU}}{\mathrm{CN}}.
\end{align}
\end{corollary}

In Proposition \ref{nurm_compare} of the next section, we use this corollary to compare the performance of regression and classification for certain choices of parameters $\psi$ and $\psi_t$.
% \begin{remark}
% This corollary demonstrates that classification consistency is achievable when a random mask augmentation sufficiently favors the true features. For example, if we fix $\psi_1$ and allow $\psi$ to change with $n$, the above bounds suggest that the conditions of \ref{thm2} are met and the risk converges to $0$ as long as $\psi$ grows sufficiently quickly. It is important to note that, in such regimes, consistency is achieved regardless of the initial spectrum of the features, so the heterogeneous random mask augmentation may perform well even when the original covariance does not admit good performance using ridge regression/Gaussian noise augmentation.
% \end{remark}
% \begin{remark}

% This corollary demonstrates that classification consistency is achievable when an augmentation sufficiently favors the true features. For example, if we fix $\psi_1$ and set $\psi = n^\alpha$, $p=n^\beta$ for some $\alpha > 0$ and $\beta > 1$, the above bounds suggest that the conditions of \ref{thm2} are met and the risk converges to $0$ as long as $\frac{\beta-1}{2} < \alpha < 2$. It is important to note that, in such regimes, consistency is achieved regardless of the initial spectrum of the features, so the heterogeneous random mask augmentation may perform well even when the original covariance does not admit good performance using ridge regression/Gaussian noise augmentation. Furthermore, this demonstrates that certain augmentation choices can be more benign for classification than regression tasks, since in this setting, we do not have $SU \to 1$, so regression is not consistent.
% \end{remark}


\subsection{Comparisons Between Regression and Classification}
The results of the previous two sections reveal several key differences between how DA affects the regression and classification tasks. Specifically, it is clear from the expressions of test error for each task that the bias of an estimator has a much more benign effect on classification than regression. We identify two key settings in which this simple difference manifests in the application data augmentation. First, we observe that it can be easier to choose augmentation parameters for classification (i.e. that a larger range of parameters can lead to favorable performance).
\paragraph{Data augmentation is easier to tune in classfication than regression.} It is observed in \cite{muthukumar2020class} that loss function is essential for measuring generalization. Specifically, they discovered that for least-squared estimator (LSE), there are cases where model generalize well
for classification task but not in regression. We complement this study by comparing the generalization with data augmentation in the two tasks. Specifically, we find that classification loss is universally upper bounded by an upper bound for the regression with the same DA, implying that regression is easier to train with DA than classification. Furthermore, we provide a concrete example using a simple DA to show that the MSE for regression is constant while POE for classification is asymptotically zero. Our findings are summarized in the following proposition.

\begin{proposition}[\textbf{DA is easier to tune in classification than regression}]\label{gen_compare}
Consider the 1-sparse model $\T^*=\sqrt{\frac{1}{\lambda_t}}\mathbf{e}_t$. Suppose the approximation error and error multiplier terms are not dominant in the bounds of Theorem \ref{gen_bound} and \ref{thm2} (simple sufficient conditions can be found in Lemma \ref{cond_tight1} and \ref{cond_tight2} in Appendix \ref{appen:lemma}) and the assumptions in the two theorem hold, then,
\begin{align}
    \mathrm{MSE}(\HT) &\lesssim %\frac{\mathbb{E}[\operatorname{Cov_g}(\x)]_{11}^2}{\lambda_t^2}
    (\lambda_{k+1}^{\text{aug}}\rho_k(\SIG_{\text{aug}};n))^2 +\left( \frac{n}{R_k(\SIG_{\text{aug}};n)} +\frac{k}{n}\right),\nonumber\\
    \mathrm{POE}(\HT) &\lesssim \sqrt{(\lambda_{k+1}^{\text{aug}}\rho_k(\SIG_{\text{aug}};n))^2 \cdot \left(\frac{n}{R_k(\SIG_{\text{aug}};n)} +\frac{k}{n}\right)\log n}.
\end{align}
So by simple inequality $x + y \geq \sqrt{xy}$, we immediately see that our upper bound for POE is less than MSE up to a log factor. As concrete examples, consider Gaussian noise injection augmentation with noise standard deviation $\sigma$ and random mask with dropout probability $\beta$ to train the 1-sparse model in the decaying data spectrum $\SIG_{ii}=\gamma^i$, $0<\gamma<1$. Let $\hat{\T}_{\text{gn}}$ and $\hat{\T}_{\text{rm}}$ be the corresponding estimators, then
\begin{align}
    \mathrm{POE}(\hat{\T}_{\text{gn}})\overset{n}{\longrightarrow} 0~~\text{while}~~\mathrm{MSE}(\hat{\T}_{\text{gn}})\overset{n}{\longrightarrow} 1,
\end{align}
as $\sigma\rightarrow \infty$. Also, when $p\log n\ll n$,
\begin{align}
    \mathrm{POE}(\hat{\T}_{\text{rm}})\overset{n}{\longrightarrow} 0~~\text{while}~~\mathrm{MSE}(\hat{\T}_{\text{rm}})\overset{n}{\longrightarrow} 1,
\end{align}
as $\beta\rightarrow 1$.
\end{proposition}
\begin{remark}
In Fig. \ref{fig:which_good}(b) and \ref{fig:which_good_cls}(b), we compare the Gaussian injection augmentation in decaying spectrum $\gamma=0.95$ for regression and classification, respectively. We observe a
sharp difference between classification and regression,
where, as we increase the Gaussian intensity, the MSE has worsen while the POE has converged to a stable value (the ratio between SU and CN stays the same), implying that a careful tuning for regression is required but is not for classification.
\end{remark}

\begin{proposition}[\textbf{Non-uniform random mask is easier to tune in classification than regression}]\label{nurm_compare}
Consider the 1-sparse model $\T^*=\sqrt{\frac{1}{\lambda_t}}\mathbf{e}_t$. Suppose the approximation error and error multiplier terms are not dominant in the bounds of Theorem \ref{gen_bound} and \ref{thm2} (simple sufficient conditions can be found in Lemma \ref{cond_tight1} and \ref{cond_tight2} in Appendix \ref{appen:lemma}) and the assumptions in the two theorems hold. Suppose we apply the non-uniform random mask augmentation as in Corollary \ref{hrm-class}. Then, if 
    $\sqrt{\frac{p}{n}} \ll \frac{\psi}{\psi_t} \ll \frac{p}{n},$ we have 

\begin{align}
    \mathrm{POE}(\hat{\T}_{\text{rm}})\overset{n, p}{\longrightarrow} 0~~\text{while}~~\mathrm{MSE}(\hat{\T}_{\text{rm}})\overset{n, p}{\longrightarrow} 1.
\end{align}

\end{proposition}
\begin{remark}
By allowing the augmentation parameters $\psi$ and $\psi_1$ to vary with $n$, the induced spectrum $\SIG_{\text{aug}}$ recovers the ``bi-level'' design which was shown in Theorem 13 of \cite{muthukumar2020class} to have separating regimes between classification and regression performance. It's worth noting that in the case where the true sparsity is known, several augmentations (including non-uniform Gaussian noise injection, which incurs no approximation error in our analysis) can give rise to the same consistency behavior described above.
\end{remark}

Secondly, we observe that the choice of augmentation itself can be more benign for classification tasks. Specifically, augmentations which are ``biased in average'' may perform similarly to their unbiased counterparts; we cannot in general expect this behavior for regression.

\textbf{Classification analysis for general biased augmentation}. As a counterpart of our regression analysis for biased estimators $\mu_g(\x) \neq \x$, we would also like to know the impact of mean bias on classification. However, the story of bias in classification is much different than that in regression since classification is less sensitive to the bias. A simple example can be seen by considering an augmentation $g(\x):=2\x$. The induced bias is $\mu_g(\x) - \x = \x$, and the trained estimator $\HT$ is just half the estimator trained with $\x$, which, however, predicts the same labels in a classification task.
Therefore, we conclude that even with a large bias, the resultant estimator might be equivalent to the original one. In fact, as we show in the next theorem, under mild conditions, the estimator is governed by the spectrum modified by the DA but rather by its mean shift.

\begin{theorem}[\textbf{POE of biased estimators}]\label{bias_cls}
    Consider the 1-sparse model $\T^*=\mathbf{e}_t$.
    and the estimator $\HT$ that solves the aERM in (\ref{DAobj}) with biased augmentation (i.e., $\mu(\x)\neq \x$).
    Assume that Assumption \ref{bias_assump} holds, and the assumptions of Theorem \ref{thm2} 
    are satisfied for data matrix $\mu(\X)$. If the mean augmentation $\mu(\x)$ modifies the $t$-th feature independently 
    of other features
    and
    the sign of the $t$-th feature is preserved under the mean augmentation transformation, i.e.,
    $\sgn\left(\mu(\x)_t\right)=\sgn\left(\x_t\right),$ $\forall \x$. Then, the POE($\HT$) 
    is simply upper bounded by,
    \begin{align}
        \mathrm{POE}(\HT)\lesssim \mathrm{POE}^o(\HT),
    \end{align}
    where $\mathrm{POE}^o(\HT)$ is any bound in Theorem \ref{thm2} with $\X$ and $\SIG$ replaced by $\mu(\X)$ and $\bar{\SIG}$, respectively.
\end{theorem}
\begin{remark}
    Note that the sign preservation is only required in mean but not in every realization of the augmentation, i.e., we only require $\E_g\left[g(\x)_t\right]$ has the same sign as $\x_t$ rather than $g(\x)_t$ has the same sign as $\x_t$ for every $g$. The latter is called the label-preserving property and has been studied in \cite{wu2020generalization} which is a much more stringent assumption. 
    From a high level perspective, the theorem tells us that as long as the signal feature preserves the sign under the mean augmentation, the scale of the generalization error is purely determined by the DA modified spectrum.
  % \vidya{If I understand right, you are saying that this condition is weaker than label-invariance, which would require the sign to be identical for every $g$. I think this is worth mentioning here with a cite to Chris Re group paper.}
\end{remark}
%\henry{integrate this subsection into 3.5}\chiraag{done}

\begin{remark}
    In Fig. \ref{fig:bvub}, we simulate the biased and unbiased random mask augmentation, and test their performances in regression and classification tasks. The setup is the 1-sparse model in the $\mathbb{R}^{128} $ ambient space with isotropic Gaussian covariate.
    For biased mask, we use the masked estimator without normalization calibration, so the augmentation mean is $
    \mu_g(\x)=(1-\beta)\x$., meaning the augmentation bias is increasing with respect to the degree of mask probability. From the figure, we see the bias can be very harmful in regression, especially in overparametrized regime ($p\leq 128$), while the performances are identical for the classification. The experiment also provides evidence for sharp different conclusions from Theorem \ref{bias-thm1} and \ref{bias_cls}.
\end{remark}

\begin{figure*}[t!]
    \centering
    \setcounter{subfigure}{0}
    \subfloat[][\footnotesize{Regression task}]{\includegraphics[width=0.5\textwidth]{imgs/reg_bvub.png}\vspace{-3mm}}
      \subfloat[][\footnotesize{Classification task}]{\includegraphics[width=0.5\textwidth]
   {imgs/cls_bvub.png}\vspace{-3mm}}
\caption{\footnotesize{{\bf \em Comparison of bias impact between regression and classification tasks} In this figure, we simulate the unbiased and biased random mask
in regression and classification tasks.
In (a), we show that the augmentation bias is mostly harmful to the regression task, especially in overparametrized regime where sample number is less or equal to $p=128$.
In (b), on the contrary, the performance is identical with and without bias in classification task. This also verifies the very different conclusions from our Theorem \ref{bias-thm1} and \ref{bias_cls}.
} \label{fig:bvub}}
\end{figure*}



% related work
%\input{files/relatedwork_v2}


% Specifically, assuming that the residual term $\Vert \HT - \BT \Vert_{\SIG}$ is lower order \chiraag{When is this true? Need a more fine-grained analysis of the error when $\psi$ is allowed to grow with $n$}, these results indicate that for regression consistency (i.e. $SU \to 1$ and $CN \to 0$), we require $\frac{\psi_1}{\psi} \ll \frac{n}{p}$. Furthermore, consistent classification is achievable even when $\frac{\psi_1}{\psi} \gg \frac{n}{p}$ as long as $\frac{\psi}{\psi_1}\sqrt{\frac{n}{p}}$ diverges in $n$. This separation between regression and classification performance is reminiscent of Theorem 13 in \cite{muthukumar2020class}, which shows such a separation for minimum norm interpolation with a ``bi-level'' covariance structure. 


==> files/convergence_assumption.tex <==
%\subsection{Convergence of empirical covariance}
%\paragraph{Comment on analysis.}
\label{sec:assump}
\eva{@henry - please merge the asmp  into analysis section as we discussed}
Although the approximate equivalence to ridge regression simplifies our analysis, there still remain technical challenges in the dependency of the implicit regularizer $\text{Cov}_G$ on the data matrix $\X$, which makes the training examples non i.i.d.
Fortunately, the dependency is weak for various data augmentations, so we can approximate $\text{Cov}_G$ with its expectation $\mathbb{E}_{\x}[\text{Cov}_g(\x)]$. On the rightmost plot in Fig. \ref{bias_var}, we have also simulated its impact on MSE to verify that this approximation error is small compared with other error components. We formalize this idea in the below assumption. In the next sections, we will showcase examples that obey the assumption.
\begin{assumption}
 \label{asm:assump1} 
We assume that augmentations are unbiased and the normalized empirical covariance converges,
    \begin{align*}
        \lim_{n\rightarrow \infty}\left\|\frac{1}{n}\mathbb{E}_{\x}[\operatorname{Cov}_g(\x)]^{-\frac{1}{2}}\sum_{i=1}^n\operatorname{Cov}_{g}(\x_i)\mathbb{E}_{\x}[\operatorname{Cov}_g(\x)]^{-\frac{1}{2}} - \I\right\| = 0.
    \end{align*}
\end{assumption}
\begin{remark}
We will show in a general proposition \ref{ind_cor} along with several concrete examples that a wide class of augmentation will satisfy this assumption in the order of $O\left(\frac{\log n}{n}\right)$. 
\end{remark}
% \vidya{I want us to comment somewhere in this section that this whole analysis would also go through for random-features regression, which is nonlinear on the data (but still can be analyzed like linear models in many cases including in the overparameterized regime). However, the effect of the same type of DA (e.g. random-masking) would be different for linear regression and random-feature regression because the induced covariance matrix $\text{Cov}_G$ will change.}

\begin{remark}
Although our model has linear dependency on data, we can elevate our framework to random-feature regression, which is linear in the feature space but has nonlinear dependency on data. 
While the basic framework of our analysis will continue to hold, the effective covariances induced by augmentations will fundamentally change.
\end{remark}


==> files/corollary20_groupinvariantaugs.tex <==
\begin{corollary}\label{cor:group-invariance}
[\textbf{Group invariance augmentation in classification tasks}]\label{gv}
Consider Gaussian covariates, i.e. $\x\sim \mathcal{N}(\mathbf{0},\SIG)$ and consider the group-invariant augmentation given by $g(\x) = \frac{1}{\sqrt{2}}\x + \frac{1}{\sqrt{2}}\x'$ (where $\x'$ is an independent copy of $\x$). Then, under the assumptions of Theorem~\ref{thm2}, the estimator induced by this augmentation has classification error given by
\begin{align}
    &\mathrm{POE}\asymp \frac{1}{2} - \frac{1}{\pi}\tan^{-1}\frac{{\mathrm{SU}}}{ {\mathrm{CN}}} , \text{ where}
    \\
    \mathrm{SU} \asymp (1-2\nu) \frac{n}{2n + {p}},~~
        &\sqrt{\frac{np}{(n+p)^2}}\lesssim \mathrm{CN} \lesssim \sqrt{(1+\mathrm{SU}^2)  \frac{np\log{n}}{(n + p)^2}}.
\end{align}
with probability at least $1-\delta-\exp(-\sqrt{n})-5n^{-1}$.
\end{corollary}
% \begin{remark}
Corollary~\ref{cor:group-invariance} evaluates a specific type of group-invariant augmentation that is reminiscent of the \emph{knockoff} model augmentation~\citep{candes2018panning}.


==> files/intro.tex <==


\section{Introduction}
Data augmentation (DA) appears in every facet of machine learning algorithms nowadays, especially in settings where data or labels are scarce \cite{shorten2019survey}. While DA can be one of the most useful components we have at our disposal, different augmentations are still applied in an ad hoc manner \cite{cubuk2019practical}, and it is often no principled understanding of how, why, and when a given DA strategy will work for a given dataset. A more grounded theoretical foundation is needed to understand and characterize the impact of augmentations in inference and to guide practice moving forward.

Recent work in building a theoretical foundation for DA has already provided insights from the group invariance \cite{chen2020group}, the effect of a single augmented sample on generalization \cite{wu2020generalization}, feature smoothing and regularization \cite{dao2019kernel} perspectives.
All these different angles provide a unique view of the impact of DA. However, to what extent different augmentation impacts the final generalization in terms of bias and variance is still not fully understood in the literature.
The answer requires a detailed analysis of how DA contributes to each component with interplays between the ground-truth model, data distribution, and augmentation distribution. 
On the other hand, modern analysis on generalization has uncovered that the data spectrum plays a key role, especially for overparameterized models where modern machine learning practices often operate \cite{bartlett2020benign,tsigler2020benign,muthukumar2020class,zou2021benign}. Nonetheless, the spectrum perspective on DA has yet to receive a comprehensive investigation, which motivates our work to perform a thorough spectral analysis on DA.

In this work, we develop a new theoretical framework for understanding the impact of DA on model generalization. It is also a simple and interpretable testbed for a new augmentation invention.
Our framework is in the context of high-dimensional linear regression and classification tasks.
Despite being simple, the linear model has shown some remarkable similarities with artificial neural network (ANN) in terms of some fundamental behaviors, which along with the amenable to interpretable analysis, makes it a good starting model to get insight. For exampl\cite{hastie2019surprises, nakkiran2020optimal, nakkiran2021deep} and benign overfitting in overparameterized regime \cite{bartlett2020benign,tsigler2020benign, zhang2021understanding} are observed in linear model and ANN. From the theoretical perspective, the neural tangent kernel theory \cite{jacot2018neural,yang2019scaling} also has shown a strong connection of ANN to the linear model.  
Our framework analyzes augmented empirical risk minimization (aERM) and shows that our framework can apply to any unbiased augmentation applied to data instances independently. As simple case studies, we also showcase how our work applied to common augmentation strategies like random mask \cite{zhong2020random, konda2015dropout} and adding Gaussian noise \cite{bishop1995training}. We develop novel generalization decompositions and derive high probability bounds for regression and classification tasks by leveraging finite analysis techniques in the benign overfitting literature. Our decomposition enables us to analyze how DA impacts the generalization in its bias and variance and provides a higher resolution on different parts of generalization error.
Our theory reveals that general DA creates effects of \textit{ridge regularization} along with \textit{data distribution manipulation} through implicit data-dependent regularization. While the ridge regularization effect always reduces the variance, the distribution manipulation could either increase or decrease bias depending on the true signal and the types of DA. Therefore, the sum effect does not always benefit the final model generalization. Also, our results highlight surprising differences in similar-seeming augmentations based on the augmentation distribution. For example, while random masking and Gaussian noise augmentation may appear to have a similar effect on breaking the information patterns in data, their effect in overparameterized regime is very different. 	For instance,  while Gaussian noise augmentation preserves the monotonicity of the original spectrum, random masking "isotropizes" data creates a non-negligible bias in the overparameterized regime.

Our framework also serves as an interpretable testbed for inventing new augmentations.
As a proof-of-concept, we propose a novel augmentation derived from the equivalence of random rotation in high dimensional space that strikes a balance between random masking in that specific randomly-selected coordinates remain unchanged but reduce bias in addition to the variance reduction offered by masking. In experiments, we find that our proposed random rotation augmentation has outstanding generalization performance on par with optimal ridge regression while remaining far more stable across its hyperparameters. 

As we perform detailed analysis in a simplified setting and make several assumptions (e.g., the population-based objective augmented-ERM approximating the augmented-SGD, etc.), we run several empirical studies to compare our theory to more practical situations that may arise.
In empirical studies, we compare our closed-form expression for aERM with augmented SGD and pre-computing augmentations in advance; We find that the latter needs significantly many augmentations to recover our analysis and has some disadvantages in terms of its generalization error. Some augmentation regimes introduce multiple descents in the test error curves. We leave the theoretical understanding of the disparity between the pre-computing and aERM as future works.

% We call that the model operates in the overparametrized regime, meaning that the model has an excessive amount of parameters that can almost perfectly fit the training data
% The overparametrization is 
% against Ockham's Razor principle
% in nature and induces too much variance in the model, causing overfitting.
% , hindering their generalization power. 
% A common remedy to the overfitting for a overparametrized model is to add strong explicit regularization to the loss of interest. This add direct penalty to the model complexity. However, modern machine learning proves to generalize well even without explicit regularization. Many \textit{implicit} regularization techniques, such as dropout, batch normalization, early stopping, or data augmentation, also lead to great success \cite{hernandez2018data}. Among them, data augmentation (DA) is prevalent in almost every facet of deep learning practice nowadays. It creates artificial training samples that virtually increase the diversity and size of the original training data.
% \henry{seems pretty weak as a beginning, i will have to think about how to rewrite it :(((}

% However, whether DA alone is enough to avoid overfitting in an overparametrized regime still remains mysterious in the literature.
% A principled theoretical understanding of why and how much it improves generalization without explicit regularization is still relatively incomplete, and key questions remain open. 
% Specifically, how data augmentation compares with explicit regularization and why does data augmentation achieve great generalization despite overfitting the noise?
% % When will data augmentation be effective for a given dataset?
% These questions have motivated our study on the model generalization with data augmentation alone in the overparametrized regime.

% % augmentations have been applied to data to generate new samples that can be used in training: the intuition is that if we can create some variations of our training data that match the expected statistics of a new test set, then this procedure can learn a mapping that will provide better generalization at test time.

% %In contrast to this popular wisdom, many procedures for DA introduce new data samples that can be significantly different from what one would expect to see in a real dataset \cite{gontijo2020affinity}. In many cases,  out-of-distribution (OOD) augmentation approaches can be quite powerful, and in many cases,  provide even better generalization than models trained with augmented samples that match the true data distribution [ref]. 
% %There is tension between finding augmentations that still match the overall data distribution while also introducing sufficient diversity into the augmented samples.
% %How and why out-of-distribution augmentation approaches work and when they will lend themselves to better generalization error, are still open questions. 

% % However, the choice of augmentation is typically done through guess and check. How and when certain classes of augmentations will perform in different signal models is still an open question. Having a universal approach for DA, or guarantees for different classes of DA, would also give practical constraints for different applied work.

% In this work, we develop a theoretical framework to address how data augmentation compares directly to explicit regularization and discover what it can recover as well as going beyond explicit regularization. We study generalization and the impact of DA on linear models for both regression and classification tasks. By leveraging the benign overfitting framework \cite{bartlett2020benign,tsigler2020benign,muthukumar2020class}, we perform a finite analysis on the augmented empirical risk minimization (aERM) \cite{chen2020group} training and mathematically characterize the generalization error covering the full spectrum from the under- to over-parametrization regime. Our work shows that the impact of DA on learning can be dissected into two important factors: (i) {\em data spectrum modification} that alters the data covariance characteristics and (ii) \rm{implicit $\ell_2$ regularization} that rectifies the spectrum condition. These are the results of the \em{implicit } and \em{data dependent} regularization DA creates, and can be characterized in closed form.
% %\henry{revised}
% %\henry{To be precise, what I mean is that DA creates an estimator of the form 
% %$\HT=(\tilde{\X}\tilde{\X}^\top + n\I)^{-1}\tilde{\X}^\top \y$, where $\tilde{\X}$ is a modified data matrix. Since data matrix $\X$ has been modified to $\tilde{\X}$, it has the effect of data distribution adaptation. Furthermore, the estimator is regularized by $n\I$ which is equivalent to ridge regression with intensity $n$. Therefore I interpret it as two separate effects.} \vidya{I understand what you are saying: I think ``data distribution adaptation" is not great as terminology - especially the word ``adaptation" as that can mean many different things. I would say it modifies the spectrum of the data covariance (and maybe also the eigenspace in some cases, e.g. non-diagonal augmentations?)}
% By establishing an analysis reduction from DA to ridge analysis \cite{tsigler2020benign}, we can directly compare the DA performance with that using explicit regularization. We further show that in some cases, data augmentation is equivalent to some well-known explicit regularization.


% % by providing an analysis of modern data augmentation techniques in terms of their ability to help improve generalization.  We dissect two important factors that DA introduces into learning: (i) {\em implicit spectral regularization} that modifies the underlying data distribution and (ii) the effect of overparameterization. We show that in some cases, we can interpret the effects of augmentations as different forms of implicit regularization on our original objective. 
% %We provide an explicit and in depth of dropout, both due to its empirical success as an augmentation in many different downstream tasks in vision (cite) as well as a wide variety of applications across different domains from text (masked language models, MLM) and audio (wav2vec) to multi-channel time-series data (azabou;  liu). Our analysis shows that XX and YY happen and we validate these effects empirically.
% %quantified in terms of its effect in interpolation of data. 
% %In the latter, the effects of augmentations can be interpreted as expansion to new parts of the space - and generation and expansion of variance in the estimator. 

% % To decompose the effects of these two different factors, we study the impact of augmentation when applied to the problem of linear regression. We derive general closed-form expressions for augmented ERM estimators and then show how we can go further to study the regularization effects of different feature-level augmentation methods (e.g., additive noise, feature dropout and masking, and mixup).  We leverage recent work in the overparameterized setting \cite{bartlett2020benign} to develop bounds on the generalization error in this case, and show how DA avoids double descent and exhibits ``benign overfitting''. 
% Our analysis reveals several helpful and harmful properties of augmentation when applied to different data models and shows the comparisons between different forms of augmentation.
%The first factor ties closely to the effects of regularization experienced  while the latter provides a benefit in the model's ability to extrapolate/ transfer to new data. 



%Our generalization bounds are for linear regression, however, much of our early analysis regarding the spectral impact of DA on the data can be applied to other loss functions and objectives as well. We show results for XX and YY, and then also confirm that our results hold in deep neural networks through a number of experiments ZZ. Through our analytical bounds on the generalization error and empirical studies of DA, we systematically answer a number of important questions that give us insight into when augmentation will be helpful vs. harmful. 

\vspace{-3mm}
\paragraph{Contributions.}~Our explicit contributions are as follows: 
\begin{itemize}
    \item We characterize generalization bounds for a broad class of augmentations, including random mask, adding Gaussian, and random rotations, for both regression and classification tasks.
    \item We identify the conditions when a specific data augmentation is helpful or harmful and when one augmentation is more favorable than the others.
    \item Empirically, we compare two augmentation strategies: the pre-computing augmentation and the augmented empirical risk minimization, and discuss the pros and cons of each method. 
    \item To the best of our knowledge, this is the first analysis that provides an explicit characterization of the effect of data augmentation in the overparameterized regime. 
\end{itemize}


==> files/regress_results_old.tex <==
f\section{Main Results}\label{analysis-results}
This section presents our theorems on the generalization performance for regression and classification tasks.
We consider estimator unbiased and biased in average separately as they exhibit significant discrepancy in generalization.
We first present a general theorem for the regression task and follow with several corollaries showcasing the application of the general theorem to some common data augmentations. Then, under further assumptions, we provide a similar set of results for the classification task, allowing us to compare how DA can behave differently for the two tasks.
Table \ref{roadmap} provides the road map to our main results in this section.
%\vidya{same comment as before about having text in between headings}
%\henry{added the lines above}

\begin{table}[ht]
\centering
\caption{\textbf{Road map of main results.}\label{roadmap}}
\setlength{\tabcolsep}{8pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.5}
\begin{tabular}[t]{|c|c|c|}
\hline
 & {\bf Regression} & {\bf Classification} \\
\hline
Meta theorem: Unbiased estimator &Theorem \ref{gen_bound}& Theorem \ref{thm2}\\\hline
Meta theorem: Biased estimator &Theorem \ref{bias-thm1}&Theorem \ref{bias_cls}
\\\hline
Case study: Random mask\henry{change}&Corollary \ref{cor_rm}, \ref{het_mask}&Corollary \ref{rm-class}, \ref{hrm-class}\\\hline
Comparisons between tasks &\multicolumn{2}{c|}{Proposition \ref{gen_compare}, \ref{nurm_compare}} \\
\hline
\end{tabular}
\end{table}%

\subsection{Preliminaries}\label{sec:gen_bound_reg}


%\vidya{I'm thinking that notation alone should come earlier --- just before Section 2.}

\subsubsection{Setup and Signal Model}
Let $\X \in\mathbb{R}^{n\times p}$ be the training data matrix with $n$ i.i.d. rows (data). Each data point $\x\in\mathbb{R}^p$ can be written as $\x = \SIG^{1/2}\z$, where $\SIG$ is a diagonal matrix with nonnegative diagonals $\lambda_i$ representing the variance of the eigen-directions, and $\z$ is a latent vector which is centered, isotropic (i.e., $\E[\z]=0$, $\mathbb{E}\left[\z\z^T\right] = \mathbf{I}$), and sub-gaussian with sub-gaussian norm $\sigma_z$. We focus our analysis on the overparameterized setting, in which $p>n$, but our analysis is also valid for $n\geq p$. 
The true data generating model is $y = \x^T\T^* +\varepsilon$, where $\varepsilon$ denotes the noise and is also isotropic and sub-gaussian with sub-gaussian norm $\sigma_{\varepsilon}$ and variance $\sigma^2$. 

% \begin{remark}
% The partition of the spectrum according to the column space of $\V$ is analogous to the partition of the first $k$ largest eigenspaces in the analysis of benign overfitting in ridge regression \cite{tsigler2020benign}. The rationale of introducing $\V$ is to accommodate for the fact that the order of data spectrum could be modified after data augmentation.
% \end{remark}

%%%%%%%%%%%%%%
\subsubsection{Error Metrics}
In this work, we will focus on the squared loss training objective \ref{DAobj} for both regression and classification. The choice is not only due to tractability but also because recent works \cite{muthukumar2020class, wang2021binary, chatterji2021finite} have shown that the squared loss can achieve competitive results when compared with cross-entropy loss in classification\footnote{We believe that our connections between DA and modified spectrum do suggest that such such equivalences could be shown in some cases for aSGD applied on the cross-entropy v.s. squared loss, but do not pursue this path in this paper.}.
%In ridge regression (or Tikhonov regularization), for example, the $R(\T)=\lambda \|\T\|_2^2$. 
For the regression task, we use the predictive mean squared error (MSE) as the metric to test the generalization power of an estimator $\hat{\T}$:
\begin{align}
    \mathrm{MSE}(\Th) = \mathbb{E}_\x[(\x^T(\hat{\T}-\T^*))^2|\X, \varepsilon],
\end{align}
where  $\theta^{\ast}$ is the true coefficient vector, $\varepsilon$ represents noise in the observed data, and $\x$ is a testing data point independent of the training data $\X$. 
For classification, we will use the probability of classification error (POE) as the testing metric:
$$\mathrm{POE}(\Th)=\mathbb{E}_\x[\mathbf{1}\{\sgn(\x^\top\Th)\neq \sgn(\x^\top\T^*)\}].$$
%Our goal is to understand the impact of data augmentations on the MSE with non-asymptotic analysis.

% For analysis, we can decompose MSE into the bias and variance components,
% \begin{align}
%     \text{MSE}\lesssim \underbrace{\|\T^*-\E_{\varepsilon}[\Th|\X]\|^2_{\SIG}}_{Bias} + \underbrace{\|\Th-\E_{\varepsilon}[\Th|\X]\|^2_{\SIG}}_{Variance}.\\
%     \underbrace{\|\T^*-\E_{\varepsilon}[\bar{\T}|\X]\|^2_{\SIG}}_{\text{Bias}} + \underbrace{\|\bar{\T}-\E_{\varepsilon}[\bar{\T}|\X]\|^2_{\SIG}}_{\text{Variance}} + \underbrace{\|\Th-\bar{\T}\|^2_{\SIG}}_{\text{Approximation Error}}\\
%     \underbrace{\|\T^*-\E_{\varepsilon}[\Th|\X]\|^2_{\SIG}}_{\text{Bias}} + \underbrace{\|\Th-\E_{\varepsilon}[\Th|\X]\|^2_{\SIG}}_{\text{Variance}}\henry{editing}
% \end{align}

\subsubsection{Spectral quantities of interest}
Recent works studying overparameterized regression and classification tasks \cite{bartlett2020benign,tsigler2020benign, muthukumar2020class, zou2021benign} have discovered that the effective ranks of the data covariance plays a central role in characterizing the generalization error. These quantities provide sufficient conditions on the data spectrum under which an overparameterized model can have good generalization; this phenomenon is termed benign overfitting. Our framework naturally inherits this principle. However, as we shall see soon, rather than depending on the effective ranks of the original spectrum, generalization depends on the \textit{augmentation modified spectrum.} In what follows, we formally define the effective ranks of the data covariance.
\begin{definition}[\textbf{Effective Rank}]\label{eff_ranks}
    For any covariance matrix (spectrum) $\SIG$ with ridge regularization intensity $c$, we define its two effective ranks as $$\rho_{k}({\SIG};c)=\frac{c+\sum_{i>k} \lambda_{i}}{n \lambda_{k+1}} ,~~R_k({\SIG};c):=\frac{(c + \sum_{i>k}\lambda_i)^2}{\sum_{i>k}\lambda_i^2}.$$
\end{definition}
%\vidya{Some of the benign overfitting math could go here; it would be well-placed.}
%\henry{the above paragraph introducing effective ranks seems a bit repetitive to Section 2.2, but i am not sure what to cut}
%\chiraag{Maybe some more discussion needed, but moved the math here}
For example, using this notation, the risk bounds for the minimum-norm least squares estimate from \cite{bartlett2020benign} can be written as,
\begin{align*}
    &\mathrm{MSE} \lesssim {\rm Bias} + {\rm Variance},\\
    &{\rm Bias} \lesssim \|\TBS\|_{\SB}^2 +  \|\TAS\|_{\SA^{-1}}^2\lambda_{k+1}^2\rho_k(\SIG ; 0)^2,~~ {\rm Variance} \lesssim \frac{k}{n} + \frac{n}{R_k(\SIG;0)},
\end{align*}
where $k < n$ is an index partitioning the spectrum into the spiked and residual parts. An interpretation of the above result is that, in order for benign overfitting, the data's spectrum should decay fast enough (small $\rho_k$) but retain a long enough tail (large $R_k$). 

Our subsequent analysis demonstrates that these quantities, applied to a modified spectrum, provide a convenient way to characterize the performance of an augmented estimator.
%%%%%%%%%%%
\subsection{A Deterministic approximation strategy for DA analysis}\label{deter_strat}
Traditional analysis decomposes MSE into the bias and variance components,
\begin{align}
    \text{MSE}\lesssim \underbrace{\|\T^*-\E_{\varepsilon}[\Th|\X]\|^2_{\SIG}}_{\text{Bias}} + \underbrace{\|\Th-\E_{\varepsilon}[\Th|\X]\|^2_{\SIG}}_{\text{Variance}}.
\end{align}
Thanks to the connection of DA estimators to ridge estimator established in the subsection \ref{impli}, we can analyze DA under the framework of ridge analysis.
However, there still remain some technical challenges to overcome: for DA, we have dependency of the implicit regularizer $\text{Cov}_G$ on the data matrix $\X$, which makes the training examples non i.i.d.
Fortunately, we can prove that the dependency is weak for various data augmentations, so we can approximate $\text{Cov}_G$ with its expectation $\mathbb{E}_{\x}[\text{Cov}_g(\x)]$.
Therefore, we propose to approximate $\Th$ using the expected augmentation covariance. Specifically,
we define the estimators:
\begin{align}\label{est_2}
    &\Th_{\text{aug}}= (\mu(\X)^T\mu(\X) + n\text{Cov}_G(\X))^{-1}\mu(\X)^Ty,\\
    &\Tb_{\text{aug}}= (\mu(\X)^T\mu(\X) + n\mathbb{E}_{\x}[\text{Cov}_g(\x)])^{-1}\mu(\X)^Ty,
\end{align}
and propose to decompose the MSE into three parts,
\begin{align}\label{decomppp}
    \text{MSE}\lesssim 
    \underbrace{\|\T^*-\E_{\varepsilon}[\bar{\T}_{\text{aug}}|\X]\|^2_{\SIG}}_{\text{Bias}} + \underbrace{\|\bar{\T}_{\text{aug}}-\E_{\varepsilon}[\bar{\T}_{\text{aug}}|\X]\|^2_{\SIG}}_{\text{Variance}} + \underbrace{\|\Th_{\text{aug}}-\bar{\T}_{\text{aug}}\|^2_{\SIG}}_{\text{Approximation Error}}.
\end{align}
The first two parts can be bounded by regression analysis with modified spectrum as the regularizer is not dependent on the data matrix $\X$, and we can separately control the error between the sample data augmentation covariance $\text{Cov}_G(\X)$ and its expectation.
We verify in Fig. \ref{bias_var}
that the approximation error is indeed non-dominant empirically. In this plot, we show the decomposition corresponding to the terms in \ref{decomppp}. We can see that the approximation error is small compared with other error components. 

\begin{figure}[h!]
    \centering
    \setcounter{subfigure}{0}
    {\includegraphics[width=1\textwidth]{imgs/bias_var_err_v2.png}\vspace{-0mm}}
    \caption{\footnotesize{\textbf{Decomposition of MSE into the bias, variance, and approximation error as in Theorem \ref{gen_bound}.} Our MSE bound is an extension of the traditional bias-variance decomposition by modifying the bias and variance terms to correspond to an estimator with a deterministic regularizer and adding an additional approximation error term to compensate for the error.
    The figures shows that the approximation error is small compared to the bias and variance ($1/10$ in the scale in this case), validating the efficacy of our proposed decomposition.}}\label{bias_var}
\end{figure}

In light of this deterministic approximation, it is convenient to introduce the following notation; denote the augmentation mean covariance, and
augmentation modified covariance,
data matrix, and model parameter as
\begin{align}
&\bar{\SIG}:=\E_\x[(\mu_g(\x)-\E_{\x}[\x])(\mu_g(\x)-\E_\x[\x])^\top]
,~{\SIG}_{aug}:=\mathbb{E}_{\x}[\text{Cov}_g(\x)]^{-1/2}\bar{\SIG}\mathbb{E}_{\x}[\text{Cov}_g(\x)]^{-1/2}, \\&\X_{aug} := \mu(\X)\mathbb{E}_{\x}[\text{Cov}_g(\x)]^{-1/2}, ~{\T}_{aug}^*:=\mathbb{E}_{\x}[\text{Cov}_g(\x)]^{1/2}\T^*,
\end{align}
respectively. Note that since the rows of $\X_{aug}$ are still i.i.d.,  $\X_{aug}$ can be viewed as a modified data matrix with covariance $\SIG_{aug}$ and $\bar{\SIG}=\SIG$ if the augmentation is unbiased in average. Since we will show that the generalization of an augmented estimator is closely related to the residual spectrum of $\SIG$, it is also convenient to define its residual kernel as $\mathcal{A}_k(\mathbf{\X}) = n\I + \mathbf{\X}\boldsymbol{P}^{\SIG}_{k:\infty}\mathbf{\X}^\top$.
We will show that approximation error is non-dominant in analysis in the next subsection.  
We will need the following assumption, which can be interpreted as a form of  law of large numbers for random matrices. 

%%%%%%%%%%%
% \include{files/convergence_assumption}
%%%%%%%%%%%
\begin{assumption}
 \label{asm:assump1} 
We assume that augmentations are unbiased and the normalized empirical covariance converges,
    \begin{align*}
        \lim_{n\rightarrow \infty}\left\|\frac{1}{n}\mathbb{E}_{\x}[\operatorname{Cov}_g(\x)]^{-\frac{1}{2}}\sum_{i=1}^n\operatorname{Cov}_{g}(\x_i)\mathbb{E}_{\x}[\operatorname{Cov}_g(\x)]^{-\frac{1}{2}} - \I\right\| = 0.
    \end{align*}
\end{assumption}
\begin{remark}
For our subsequent results to be meaningful, it is further required that this convergence is sufficiently fast as $n, p \to \infty$ (we will generally assume that $p$ is polynomial in $n$). We will show in a general proposition \ref{ind_cor} and with several concrete examples that a wide class of augmentations will satisfy this assumption in the order of $O\left(\frac{\log n}{n}\right)$. We will see that this rate is sufficient for our results to be tight in non-trivial regimes\textemdash specifically, whenever this approximation error decays quickly with respect to the bias and variance.
\end{remark}
% \vidya{I want us to comment somewhere in this section that this whole analysis would also go through for random-features regression, which is nonlinear on the data (but still can be analyzed like linear models in many cases including in the overparameterized regime). However, the effect of the same type of DA (e.g. random-masking) would be different for linear regression and random-feature regression because the induced covariance matrix $\text{Cov}_G$ will change.}

\begin{remark}
Although our model has linear dependency on data, we can elevate our framework to random-feature regression, which is linear in the feature space but has nonlinear dependency on data. 
While the basic framework of our analysis will continue to hold, the effective covariances induced by augmentations will fundamentally change.
\end{remark}

%\henry{comnent on the rate of p}\chiraag{done}


\subsection{Regression analysis}\label{regress-results}

With the connection of DA to ridge regression in \ref{impli} and the deterministic approximation method in \ref{deter_strat}, we are ready to present our generalization analysis of regression task for data augmentation estimators.The results for the unbiased estimators in average are presented in subsection \ref{unbias_regress}, and biased estimators are in \ref{bias_regress}.
\subsubsection{Regression analysis for general classes of unbiased augmentations}\label{unbias_regress}
In this subsection, we present the general theorem for unbiased estimators in average i.e., $\mu(\X)=\X$ in 
Theorem \ref{gen_bound}. Then we provides several corollaries to showcase the use of it.  All proofs in this section can be found in Appendix \ref{main_proof_reg}.

\begin{theorem}[\textbf{High probability bound of MSE for unbiased DA}]\label{gen_bound} 
    Consider an unbiased data augmentation $g$ and its estimator $\theta_{\text{aug}}$. Denote \footnote{We suppress the dependency of $\boldsymbol{\Delta}_g$ on the data $\X$ for notation simplicity.}
    $$\boldsymbol{\Delta}_G := \big\|\mathbb{E}_{\x}[\operatorname{Cov}_g(\x)]^{-\frac{1}{2}}\operatorname{Cov}_G(\X)\mathbb{E}_{\x}[\operatorname{Cov}_g(\x)]^{-\frac{1}{2}}-\I\big\|,$$ and $\kappa$ the condition number of $\SIG\mathbb{E}_{\x}[\operatorname{Cov}_g(\x)]^{-1}$. Assume with probability $1-\delta'$, we have that the condition numbers for the matrices $\mathcal{A}_{k_1}(\mathbf{\X_{\text{aug}}})$, $\mathcal{A}_{k_2}(\mathbf{\X_{\text{aug}}})$ are bounded by $L_1$ and $L_2$ respectively, and  $\boldsymbol{\Delta}_G\leq c'$ for some constant $c' < 1$. 
    Then, there exist some constants $c,~ C$ depending only on $\sigma_x$ and $\sigma_\varepsilon$, such that, with probability $1- \delta'-3n^{-1}-\exp(-ct)$, the testing MSE is bounded by
    \begin{align*}
      \big|\mathrm{MSE}&-({\color{blue}\mathrm{Bias}} + {\color{red}\mathrm{Variance}})\big|~\lesssim~  {\color{olive}\mathrm{Approximation Error}},\nonumber\\
      \frac{{\color{blue}\mathrm{Bias}}}{C_xL_1^4} ~\lesssim &~
        {{\left(\left\|\mathbf{P}^{\SIG_{\text{aug}}}_{k_1+1:p}{\theta}_{\text{aug}}^{*}\right\|_{\SIG_{\text{aug}}}^{2}
      +\left\|\mathbf{P}^{\SIG_{\text{aug}}}_{1:k_1}{\theta}_{\text{aug}}^{*}\right\|_{\SIG_{\text{aug}}^{-1}}^{2}\frac{(\rho^{\text{aug}}_{k_1})^2}{{(\lambda^{\text{aug}}_{k_1+1})^{-2}}+(\lambda^{\text{aug}}_{1})^{-2}(\rho^{\text{aug}}_{k_1})^2}\right)}}, \nonumber\\
        \frac{{\color{red}\mathrm{Variance}}}{\sigma_{\varepsilon}^{2} tL_2^2\Tilde{C}_x}~\lesssim&~{{ \left(\frac{k_2}{n}+ \frac{n}{R^{\text{aug}}_k}\right)}},~~{{\color{olive}\mathrm{Approx. Error}}}~\lesssim~\kappa^{\frac{1}{2}}\boldsymbol{\Delta}_G \left(\|\T^*\|_{\SIG} +  \sqrt{\mathrm{Bias} + \mathrm{Variance}}\right),
    \end{align*}
    where $\rho^{\text{aug}}_{k}:=\rho_{k}(\SIG_{\text{aug}};n)$ and $R^{\text{aug}}_{k}:=R_{k}(\SIG_{\text{aug}};n)$.
    % Furthermore, we have the lower bound
    % \[
    %     \mathrm{MSE} \gtrsim \mathrm{MSE}(\BT) - {\color{olive}\mathrm{Approximation Error}}.
    % \]
    Finally, assume the condition number of $\SIG_{\text{aug}}$ is bounded by $L$ and $k_i$ is chosen such that $\frac{1}{L} > C\sqrt{\frac{n}{p-k_i}}+\frac{t}{\sqrt{p-k_i}}$
    where $C$ is some constant depending solely on $\sigma_x$ then there exists another constant $c$ such that with probability $1-\exp(-2ct^2)$,
    \begin{align}\label{l_bound}
        {L}_{i} \leq \frac{n + {\lambda}^{\text{aug}}_1\left(1 + C\sqrt{\frac{n}{p-k_i}}+\frac{t}{\sqrt{p-k_i}}\right)}{n + {\lambda}^{\text{aug}}_1\left(\frac{1}{L} - C\sqrt{\frac{n}{p-k_i}}-\frac{t}{\sqrt{p-k_i}}\right)}\leq \max\left(1, \frac{1 + C\sqrt{\frac{n}{p-k_i}}+\frac{t}{\sqrt{p-k_i}}}{\frac{1}{L} - C\sqrt{\frac{n}{p-k_i}}-\frac{t}{\sqrt{p-k_i}}}\right),~\forall i \in {1,2}.
    \end{align}
    \end{theorem}
% \begin{remark}[Magnitude of the error term $\|\hat{\T}_{\text{aug}}-\BT\|^2_\SIG$]
%     From the above derivations, we deduce that as long as $\mathbb{E}_{\x}[\text{Cov}_g(\x)]=c'$ for some constant $c'>0$ and $\boldsymbol{\Delta}_g = o(n)$ then the term is vanishing with respect to $n$. We will see soon in the below corollaries that the conditions hold for many augmentations.
% \end{remark}



\paragraph{When is our bound in Theorem \ref{gen_bound} tight?}
There is a natural question of whether our bound in Theorem \ref{gen_bound} is tight. The tightness of the testing error to an estimator with data independent regularizer is established in Theorem 5 of \cite{tsigler2020benign}. Hence, as long as the approximation error in our theorem is dominated by either bias or variance then our bound will be tight too. Roughly speaking this happens when the convergence of $n^{-1}\text{Cov}_G(\X)$ to $\mathbb{E}_{\x}[\text{Cov}_g(\x)]$  is sufficiently fast with respect to $n$. More precisely, $\|\text{Cov}_G(\X)-\mathbb{E}_{\x}[\text{Cov}_g(\x)]\|\lesssim \left(\sqrt{\mathrm{Bias}} + \sqrt{\mathrm{Variance}}\right)$. 
For interested readers, we have include the full technical  condition in Lemma \ref{cond_tight1} of Appendix \ref{appen:lemma}.

We showcase how to use Theorem \ref{gen_bound} for various data augmentations in a series of corollaries. An important class of augmentation in practice is where the augmentations are done independently in the features. This class subsumes many prevailing augmentations like random mask, salt-and-pepper, and Gaussian noise injection. Because the augmentation covariance $\text{Cov}_g(\x)$ is diagonal for DA in this class, we can simplify Theorem \ref{gen_bound} into the next proposition. The proposition shows that this class of augmentation has a reordering effect on the feature importance.  
\begin{proposition}[\textbf{Independent Feature Augmentations}]\label{ind_cor}
    Let $g$ be an independent feature augmentation,
    and $\pi: \{1,2,\dots,p\}\rightarrow \{1,2,\dots,p\}$ be the function that maps the original feature index to the sorted index according to the eigenvalues of ${\SIG}_{\text{aug}}$ in a non-increasing order, then data augmentation has a spectrum reordering effect which changes the MSE through the bias modification:
\begin{align*}
    \frac{\text{Bias}}{C_xL_1^4}&\lesssim 
       \left\|{\theta}^{*}_{\pi(k_1+1:p)}\right\|_{{\Sigma}_{\pi(k_1+1:p)}}^{2}
    +\left\|{\theta}_{\pi(1: k_1)}^{*}\right\|_{\mathbb{E}_{\x}[\text{Cov}_g(\x)]^2{\Sigma}_{\pi(1: k_1)}^{-1}}^{2}\frac{(\rho_{k_1}^{\text{aug}})^2}{{(\lambda^{\text{aug}}_{k_1+1})^{-2}}+(\lambda^{\text{aug}}_{1})^{-2}(\rho_{k_1}^{\text{aug}})^2},
\end{align*}
where $\pi(a:b)$ denotes the indices of $\pi(a),\pi(a+1),\dots,\pi(b)$.
Furthermore, if the variance of feature augmentation $\operatorname{Var}_{g_i}(g_i(x))$ is a sub-exponential random variable with sub-exponential norm $\sigma_i^2$ and mean $\bar{\sigma}_i^2$, $\forall i \in \{1,2,\dots,p\}$, and $p=O(n^{\alpha})$ for some $\alpha >0$, then there exists constant $c$, depending only on $\alpha$, such that with probability $1-n^{-3}$, 
\begin{align*}
    \boldsymbol{\Delta}_{G}\lesssim  \max_i\left(\frac{\sigma_i^2}{\bar{\sigma}_i^2}\right)\frac{\log n}{n}.
\end{align*}
\end{proposition}

%A concrete application of this bound to a feature dependent augmentation is the rotation in random plane where we have
%$$\mathrm{Cov}_G(\X)=\frac{4(1-\cos \alpha)}{np}\left(
%    \operatorname{Tr}\left(\X^\top\X\right)\I - \X^\top\X\right),~~\boldsymbol{\Delta}_{G}\lesssim  \frac{\lambda_1n +\sum_j\lambda_j}{n\sum_{j>1}\lambda_j}.$$
%We provide the detailed derivation in Appendix \ref{non_diag}.

\subsubsection{Examples of independent feature augmentations}
In this subsection, we apply Proposition \ref{ind_cor} to specific augmentation strategies and analyze their MSE performances.

First, note that our Proposition \ref{ind_cor} generalizes and recovers the existing bounds on ridge and ridgeless estimators \cite{bartlett2020benign,tsigler2020benign}. The connection is that ridge and ridgeless estimators are equivalent to Gaussian noise injection \cite{bishop1995training} and its limit, so our propositions applies. For self-contained, we include their generalization bounds by our theorem in Appendix \ref{pf_reg_cor}.

Next, we consider the popular random mask augmentation, in which certain coordinates of each data vector are set to $0$ with a given probability. This type of augmentation has been widely used in various machine practices \cite{he2022masked, konda2015dropout}, and is a simplified version of the popular cutout augmentation \cite{devries2017improved}. Its idea is similar to the dropout training in neural networks \cite{bouthillier2015dropout}. The subtle difference between random mask and dropout is that one is done in the input space, and the other is in the feature space. In either case, it provides implicit regularization and is extremely easy to implement. 

\begin{corollary}[\textbf{Generalization of random mask augmentation}]\label{cor_rm}
    Consider the unbiased random mask augmentation $g(\x) = [b_1\x_1,\dots,b_p\x_p]/(1-\beta)$, where $b_i$ are i.i.d. Bernoulli(1-$\beta$). Define $\psi=\frac{\beta}{1-\beta}\in [0, \infty)$. The estimator can be expressed in a closed-form as $\Th=(\X^T\X+\psi\text{diag}(\X^T\X))^{-1}\X^T\y$. Let $L_1$, $L_2$, $\kappa$, $\delta'$ be defined as in Theorem \ref{gen_bound}, and assume $\SIG$ is diagonal. Then for any set $\mathcal{K}\subset \{1,2,\dots,p\} $ consisting of $k_1$ elements, there exists some constant $c'$, which depends solely on $\sigma_z$ and $\sigma_{\varepsilon}$, such that with probability $1-\delta'-3pn^{-5}$, the generalization error is upper bounded by
    \begin{align*}
        \mathrm{MSE} \lesssim& 
       \underbrace{\left\|{\theta}^{*}_{\mathcal{K}}\right\|_{{\Sigma}_{\mathcal{K}}}^{2}
        +\left\|{\theta}_{\mathcal{K}^c}^{*}\right\|_{{\Sigma}_{\mathcal{K}^c}}^{2}\frac{(\psi n + p - k_1)^2}{n^2 + (\psi n + p -k_1)^2}}_{\mathrm{Bias}}\\
        +& \underbrace{\frac{k_2}{n}+\frac{ n(p-k_2)}{(\psi n + p - k_2)^2}}_{\mathrm{Variance}}
        +\underbrace{ \frac{\sigma_z^2\log n}{n}\|\T^*\|_{\SIG}}_{\mathrm{Approx. Error}}.
    \end{align*}
\end{corollary}
\begin{remark}[\textbf{Effect of random mask on the bias and variance}]
    From the previous corollary, together with the fact that $\psi=\frac{\beta}{1-\beta}$ is monotonically increasing with mask intensity, we found that the bias is increasing with respect to the mask intensity while variance is the opposite. This insight from the bound illustrates the general pulling effects of data augmentations on the overall MSE: data augmentation mitigates the variance at the cost of bias increase. Fig. \ref{bias_var} illustrates these observations.
\end{remark}

We next consider a popular ``salt-and-pepper'' style augmentation in which each coordinate is replaced by random noise with given probability and is retained otherwise. We note that, like many augmentations used in practice, this augmentation is an example of a \textit{composition} of two other common augmentations (in this case, random mask and Gaussian noise injection).
\begin{corollary}[
\textbf{Generalization of Pepper/Salt augmentation}]\label{salt_cor}
    Consider the pepper/salt augmentation which modifies the data by $g(\x) = [\x'_1,\dots,\x'_p]$, where 
    $\x'_i=\x_i/(1-\beta)$ with probability $1-\beta$ and otherwise $\x_i'=\mathcal{N}(\mu,\sigma^2)/(1-\beta)$. 
    The pepper augmentation, 
    which has $\mu=0$, is an unbiased estimator. So an application of Theorem \ref{gen_bound} gives the upper bound of MSE as, 
    \begin{align*}
        \mathrm{Bias}&\lesssim 
        \left\|{\theta}^{*}_{k+1:p}\right\|_{{\Sigma}_{k+1:p}}^{2}
        +\left(\frac{1+\alpha^{-1}}{\sigma^2(1+\psi)}\right)^2\left\|{\theta}_{k+1:p}^{*}\right\|_{{\Sigma}_{1:k}}^{2}\rho_k^2(\SIG;\psi(1+\psi)\sigma^2 n),\\
        \mathrm{Variance}&\lesssim \frac{k}{n}+\frac{n(1+\alpha)^2}{R_k(\SIG;\psi(1+\psi)\sigma^2n(1+\alpha))},\\
        \mathrm{Approx. Error}&\lesssim \frac{\log n}{n}\frac{\sigma_x^2\lambda_1\kappa^{\frac{3}{2}}}{\lambda_1 + \sigma^2\kappa(1+\psi)}\|\T^*\|_{\SIG},
    \end{align*}
    where $\psi=\frac{\beta}{1-\beta}$, $\alpha$ is some parameter and $k$ is chosen such that $\lambda_i=\arg\max\limits_i\{\lambda_i > \frac{\sigma^2}{1-\beta}\}$.
\end{corollary}

\paragraph{When is data augmentation helpful?}
Before closing our investigation on estimators which are unbiased in average, 
we want to ask the final question: what is the interplay of data augmentation with the true model? To demonstrate that our theorem can help extract insights for answering this question, we use a non-uniform random mask scheme as a case study. Specifically, we consider the $k$-sparse model where $\T^* = \sum_{i\in\mathcal{I}_{\mathcal{S}}}\alpha_i\mathbf{e}_i$ and $|\mathcal{I}_{\mathcal{S}}|=k$. Define the mask parameter $\psi:=\frac{\beta}{1-\beta}$ where $\beta$ is the dropout rate. Suppose we employ non-uniform mask: $\psi_i=\psi_1$ if $i \in \mathcal{I}_{\mathcal{S}}$ and $=\psi_0$ otherwise. Conceptually, a good mask should retain the semantics from the original data as much as possible while masking the irrelevant parts. We can study this principle analytically through the generalization bound. A full characterization can be found in the Appendix.

\begin{corollary}[\textbf{Non-uniform random mask in $k$-sparse model}]\label{het_mask} Consider the $k-$sparse model. Suppose we employ non-uniform random mask where $\psi=\psi_1$ if $i\in \mathcal{I}_{\mathcal{S}}$ and $=\psi_0$ otherwise. Then, if $\psi_1 \leq \psi_0$, we have
\begin{align*}
    &\mathrm{Bias} \lesssim  \frac{\left(\psi_{1}n + \frac{\psi_{1}}{\psi_{0}}\left(p-|\mathcal{I}_{\mathcal{S}}|\right)\right)^2}{n^2 + \left(\psi_{1}n + \frac{\psi_{1}}{\psi_{0}}\left(p-|\mathcal{I}_{\mathcal{S}}|\right)\right)^2}\|\T^*\|_\SIG^2,~~
    \mathrm{Variance} \lesssim \frac{|\mathcal{I}_{\mathcal{S}}|}{n} + \frac{n\left(p - |\mathcal{I}_{\mathcal{S}}|\right)}{\left(\psi_0 n + p - |\mathcal{I}_{\mathcal{S}}|\right)^2},\\
    &\mathrm{Approx. Error} \lesssim \sqrt{\frac{\psi_1}{\psi_0}}\frac{\sigma_z^2\log n}{n}\|\T^*\|_{\SIG},
\end{align*}
while if $\psi_1 > \psi_0$ then,
\begin{align*}
    \mathrm{Bias} \lesssim  \|\T^*\|_\SIG^2,~~\mathrm{Variance} \lesssim \frac{\left(\frac{\psi_1}{\psi_o}\right)^2 + \frac{|\mathcal{I}_{\mathcal{S}}|}{n}}{\left(\frac{\psi_1}{\psi_o}+\frac{|\mathcal{I}_{\mathcal{S}}|}{n}\right)^2}, ~~\mathrm{Approx. Error} &\lesssim \sqrt{\frac{\psi_0}{\psi_1}}\frac{\sigma_z^2\log n}{n}\|\T^*\|_{\SIG}
\end{align*}
\end{corollary}

% The non-uniform random mask also has a diagonal augmentation covariance with diagonal element $\text{Cov}_G(\X)_{ii} = \frac{1}{n}\psi_i (\X^T\X)_{ii}$, $\psi_i=\frac{\beta_i}{1-\beta_i}$. Using a simple extension of Corollary \ref{ind_cor}, we can bound the bias and variance by
% \begin{align}
%     \text{Bias} \lesssim \frac{(\psi_1n + \frac{\psi_1}{\psi}(p-k_1))^2}{n^2 + (\psi_1n + \frac{\psi_1}{\psi}(p-k_1))^2},~\text{Variance} \lesssim \frac{k_2}{n} + \frac{n(p-k_2)}{(\psi n + p - k_2)^2}.
% \end{align}
We can see that bias is decreasing the mask ratio $\psi_1/\psi$ between signal part ($\mathcal{I}_{\mathcal{S}}$) and noise part decreases. This corroborates the idea that a successful augmentation should retain semantic information as compared to the noisy parts of the data. We note that the bound has a sharp transition---if we mask the signal more than the noise, the bias bound becomes proportional to the performance of a null estimator. While the previous augmentations mentioned generally experience a tradeoff between bias and variance as the augmentation intensity increases, we observe that the non-uniform random mask can reduce both bias and variance with appropriate parameter selection. However, while offering useful insight, this scheme relies crucially on knowledge of the target signal's sparsity and may be of limited practical interest. Next, we describe a technique for analyzing augmentations which do not act independently on each coordinate and give a concrete example of how such an augmentation can yield favorable performance \textit{without} such oracle knowledge. 

\paragraph{Analysis for dependent feature augmentation.} Proposition
\ref{ind_cor} gives the bound for the approximation error for independent feature augmentation, where $\boldsymbol{\Delta}_{G}\lesssim \frac{\log n}{n}$. However, one might wonder whether the error is still vanishing for dependent augmentation. While the result is case by case and we don't have a guarantee for a general dependent augmentation, we do believe that the error is small when the augmentation dependency between features is weak. Specifically, to bound the error for a dependent augmentation, we propose the decomposition $\mathrm{Cov}_G(\X)=\D + \Q$, where $\D$ is a diagonal matrix representing the \textit{independent} feature augmentation part. Then, we have
\begin{align*}
    \boldsymbol{\Delta}_{G}\lesssim \frac{\|\D-\E\D\| + \|\Q-\E\Q\|}{\mu_p(\E_\x\mathrm{Cov}_g(\x))}.
\end{align*}
In this way, even the error of non-diagonal part $\|\Q-\E\Q\|$ resulting from dependent feature augmentation is usually large, it can be canceled out by the denominator $\mu_p(\E_\x\mathrm{Cov}(\x))$ as long as $\E_\x\mathrm{Cov}(\x)$ is well-conditioned. We provide an example of how this approach can provide informative bounds in the next section.

\subsection{Using our framework as new testbed for DA}

%With techniques from high dimensional statistics, we can derive an approximation to the estimator and apply our theorem to estimate its generalization. 
Our framework can be used as a testbed for quick check of a new DA's generalization.
As a proof-of-concept, and as an example of a dependent augmentation,
we analyze the novel DA introduced in Section \ref{sec:rot}.
The properties of this rotation in terms of its generalization can be described in the following corollary. The derivation of the estimator and the proof of the corollary are deferred to Appendix \ref{common_est}. Using the technique from the previous section, the approximation error can also be shown to decay approximately as $O\left(\frac{1}{n} \right)$ (proof provided in Appendix \ref{non_diag}).
\begin{corollary}[\textbf{Generalization of random rotation}]\label{rot}
    The estimator from rotation in random plane with angle $\alpha$ can be expressed as $$\hat{\T}_{\text{rot}} = \left(\X^\top\X + \frac{4(1-\cos \alpha)}{p}\left(
    \operatorname{Tr}\left(\X^\top\X\right)\I - \X^\top\X\right)\right)^{-1}\X^\top \y.$$
    Applying Theorem \ref{gen_bound}, we can deduce that 
    \begin{align*}
        \mathrm{Bias}(\hat{\T}_{\text{rot}}) \asymp \mathrm{Bias}(\hat{\T}_{\text{lse}}),
    \end{align*}
    for sufficiently large $p$ (overparametrized regime), and the variance is bounded by
    \begin{align*}
        \mathrm{Var}(\hat{\T}_{\text{rot}})\lesssim \mathrm{Var}(\hat{\T}_{\text{ridge,}\lambda}),
    \end{align*}
    where $\hat{\T}_{\text{lse}}$ and $\hat{\T}_{\text{ridge,}\lambda}$ denote the least squared estimator and ridge estimator with ridge intensity $\lambda = {np^{-1}(1-\cos\alpha)\sum_{j}\lambda_j}$.
\end{corollary}
\begin{remark}
    Surprisingly through our analysis, our proposed simple data augmentation strategy leads to an estimator not only having the best asymptotic bias matching LSE, but also inheriting the merit of variance reduction like a ridge regression. Our experiments in Fig \ref{fig:which_good} and \ref{fig:which_good_cls} has further showcased its good performance and robustness.
%    \vidya{Rather than ``matching LSE", I think what you want to say is that there is an explicit improvement even over LSE because of modified spectrum. And ideally we do include a few examples here.}
 %   \henry{actually the bias is not really better than LSE but rather in the same scale w.r.t. $n$. I dont know if its even possible to get better bias than LSE without knowledge of the true model tho...}
\end{remark}
%\vidya{Comment on the surprise of being able to find an augmentation that reduces both bias and variance.}\henry{done}

% \vidya{Addition below for a more general biased DA}
\subsubsection{Regression analysis for general biased augmentations in average}\label{bias_regress}

The expressions in the previous section and ensuing equivalence to ridge regression (in the MSE) assume that the augmentation is \emph{unbiased in average}, i.e. that $\mu_g(\x) = \x$.
We now derive and interpret the expression for the estimator that is induced by a general augmentation that can be biased.

For convenience, we introduce following additional definitions.
\begin{definition}
    We define the bias and bias covariance induced by the augmentation $g$ as 
    \begin{align}
        \delta(\x) := \mu_g(\x) - \x,~~\operatorname{Cov}_{\delta}:=\mathbb{E}_\x\left[\delta(\x)\delta(\x)^\top\right].
    \end{align}
\end{definition}

Since $\delta(\x)$ is not zero for a biased augmentation, we lose the exact equivalence to an ridge regression as in (\ref{simt}), as there is an induced covariate-shift in the training data that does not appear in the test data. This results in two sources of generalization errors. Firstly, the equivalent testing data has a covariance mismatch with training data: the former has covariance ${\text{Cov}_G}^{-1/2}\SIG{\text{Cov}_G}^{-1/2}$ while the latter has ${\text{Cov}_G}^{-1/2}\bar{\SIG}{\text{Cov}_G}^{-1/2}$. Secondly, there is observation covariate mismatch, where our observations are from $\X\T^*$ rather than $\mu(\X)\T^*$.
Our next generalization result for biased estimators reflects these two factors explicitly, and is a strict generalization of Theorem \ref{gen_bound}. To facilitate the analysis, we impose the following assumption.
\begin{assumption}\label{bias_assump}
    For the input data $\x$, the mean transformation $\mu(\x)$ admits the form of $\mu(\x)=\bar{\SIG}\bar{\z}$, where $\bar{\SIG}$ is some covariance matrix and $\bar{\z}$ is a centered and isotropic sub-gaussian vector with sub-gaussian norm $\sigma_{\bar{x}}$.  
\end{assumption}

Now we are ready to state our theorem for biased estimator. The proof is deferred to Appendix \ref{main_proof_reg}.
\begin{theorem}[\textbf{Bounds on the MSE for Biased Augmentations}]\label{bias-thm1}
Consider the estimator $\HT$ obtained by solving the aERM in (\ref{DAobj}) with biased augmentation (i.e., $\mu(\x)\neq \x$).
Denote $\mathrm{MSE}^o(\HT)$ the unbiased MSE bound in Theorem \ref{gen_bound} with $\SIG$ replaced by $\bar{\SIG}$, and the augmentation bias convergence error  $${\Delta}_\delta:=\left\|\frac{(\mu(\X)-\X)^\top(\mu(\X)-\X)}{ n}-\operatorname{Cov}_{\delta}\right\|.$$ Suppose the assumptions in Theorem \ref{gen_bound} hold for the mean augmentation $\mu(\x)$ .
Then, with probability $1- \delta'-3n^{-1}-\exp(-ct)$ we have,
\begin{align*}
    \mathrm{MSE}(\HT)\lesssim\left(1 + \|\SIG^{\frac{1}{2}}\bar{\SIG}^{-\frac{1}{2}}-\I\|\right)^2\left(\sqrt{\mathrm{MSE}^o(\HT)} + \sqrt{\frac{\|\bar{\SIG}\D^{-1}\|}{\lambda_1^{\text{aug}}}}(1+{\Delta}_G)\left(\sqrt{\Delta_\delta}\|\T^*\|+\|\T^*\|_{\operatorname{Cov}_{\delta}}\right) \right)^2.
\end{align*}
where $\D = \E_x[\operatorname{Cov}_g(\x)]$.
\end{theorem}
\begin{remark}
    When the estimator is unbiased, we have: 1. $\|\SIG^{\frac{1}{2}}\bar{\SIG}^{-\frac{1}{2}}-\I\|=0$; this term arises from the testing distribution mismatch. 2. ${\operatorname{Cov}_\delta} =\|\boldsymbol{\Delta}_1\|=0$; these terms arise from the training observation distribution mismatch. Thus, we see the bound has reduced to $\mathrm{MSE}^o(\HT)$ when $g$ is unbiased. 
\end{remark}
\begin{corollary}[\textbf{Generalization of biased mask augmentation}]\label{bias_mask}
    Consider the biased random mask augmentation $g(\x) = [b_1\x_1,\dots,b_p\x_p]$, where $b_i$ are i.i.d. Bernoulli(1-$\beta$). Define $\psi=\frac{\beta}{1-\beta}\in [0, \infty)$. Assume the assumptions in Corollary \ref{cor_rm} hold. Then  with probability $1-\delta'-3pn^{-5}$, the generalization error is upper bounded by 
    \begin{align*}
        {\mathrm{MSE}(\HT)}\leq \left(\sqrt{\mathrm{MSE}^o} + \psi\left(1+\frac{\log n}{n}\right)\cdot\left(\left(\lambda_1 + \frac{\sum_{j}\lambda_j}{n}\right)\|\T^*\|+\|\T^*\|_{\SIG}\right) \right)^2,
    \end{align*}
    where $\mathrm{MSE}^o$ is the bound given in Corollary \ref{cor_rm}.
\end{corollary}
\begin{remark}
    We see clearly that the generalization increases as the mask probability increases ($\psi$ increases from $0$ to $\infty$), and when the bias is small it approaches to the unbiased performance. We also verify this bound in Fig. \ref{fig:bvub}.
\end{remark}
% \henry{This result is a strict generalization to Theorem \ref{gen_bound} so it should be moved to later sections. Here is just a temporary placeholder. As explained in the remark, i think this bound can be generalized to domain shift problem too.}

%\begin{remark}[Comparison to Interpolation]\henry{add some comments from experiments for comparisons}
%In comparison to the MNI, where the vanishing variance can only be achieved by certain spectrum, it is always achievable with dropout augmentation for any finite dimensional model.
%The price is the bias might be larger than an interpolator. However, as the expression has shown, the bias could be controlled by adjusting the dropout parameter by assuming a small norm on the optimal parameter.
%\end{remark}



% \subsection{Discussion and connections to previous work}


% Talk about how to interpret the bounds. How can you place these results in the context of other work?

==> files/relatedwork_v2.tex <==
% \subsection{Comparisons with Related Work}
%\vidya{This is a weird place to put related work. We should either do it after our contributions or in appendix (I tend to prefer the format unless we're space-constrianed).} \eva{how about this?}

% Recent work in building a theoretical foundation for DA has provided insights into the invariance properties induced by structured group-level (rotation, translation) augmentations \cite{chen2020group}, the effect of instance specific augmentation on generalization \cite{wu2020generalization}, and kernel theory that links DA to kernel classifier \cite{dao2019kernel}. 
% The authors in \cite{chen2020group} propose a framework based on the group theory and explain that the averaging effect helps the model generalize in variance reduction.
% However, in terms of bias estimation, as they assume the data distribution is approximately invariant after augmentation, their estimation for augmentation with significant distributional shift is limited. On the other hand, our work significantly relaxes the assumption by only requiring the augmentation invariant in the mean. The authors have studied the generalization in the overparameterized regime for neural networks, but it can only apply to DA with discrete states. 

% \cite{dao2019kernel} proposes a Markov process-based framework to model the DA and builds up a close connection between DA and a kernel classifier generated from the underlying augmented data distribution.
% Under their model, they observed data dependent regularization induced by DA. However, their observations hold only when the feature map is not significantly modified by DA, while our regularization characterization is exact. They have analyzed an aERM type of objective with a more general loss and augmentation process, and provided an explanation of the variance reduction and feature averaging effect of DA, but they lose the tractability of the generalization error. With a simpler model in our work, we can provide tight generalization error estimation for a broad class of data augmentation.

% The most closely related work to ours is \cite{wu2020generalization} which studies the linear model generalization with DA for regression in overparametrized regime. They analyze the effect of instance-specific augmentation and do not capture the random nature of augmentation. In our work, we show that the covariance of augmentation plays an essential role in regularization and data distribution manipulation that cannot be observed without modeling the randomness of the augmentation. We both study the class of label invariant augmentation, where only covariate is modified. They find that this class of augmentation has the effect of enlarging the span of training data. However, their conclusion relies on assuming the output of the true model is invariant with respect to the augmentation, which hardly held in general for a linear model. Our work does not require such restrictions. The work also studies the generalization bound, but their bound is finite only when the estimator is explicitly regularized, while our work can be applied to no explicit regularized estimator to get the sole effect of data augmentation.
% Finally, their work applies only to regularized estimators; hence the alone effect from DA entangles with explicit regularization, but our works can apply to regularized or unregularized cases.

% Recently, \cite{shen2022data}  investigates  DA from a dynamic perspective for a two-layer convolutional neural network, and by assuming a permutation-alike augmentation, they find the feature manipulation effect of DA that unfolds during the learning procedure, where DA enables the model to better learn the essential feature for a classification task. They also observe that the benefit becomes more pronounced for nonlinear models. Our work is also coherent with their observations that data manipulation effect plays a key role in generalization and learning: dominant features with higher variance can be either suppressed or enhanced by different augmentation and have different impacts on the model generalization. While they have great insights from the learning dynamics and nonlinear networks that we haven't yet studied under our framework, we see the nonlinear models discussed in their work an important next step. At the same time, we provide an analysis for a wider class of augmentations and provide a  general framework to understand all of these strategies under same lens. In contrast, our focus is on a very general class of augmentations in the simplest situation for overparameterization. We believe that combining our insights with a more complex nonlinear model analysis is a great future direction.

==> files/tuningDA_regvsclass.tex <==
\begin{proposition}[\textbf{DA is easier to tune in classification than regression}]\label{gen_compare}
Consider the 1-sparse model $\T^*=\sqrt{\frac{1}{\lambda_t}}\mathbf{e}_t$ for Gaussian covariate with independent components and an independent feature augmentation. Suppose that the approximation error is not dominant in the bounds of Theorem \ref{gen_bound} (simple sufficient conditions can be found in Lemma \ref{cond_tight1} in Appendix \ref{appen:lemma}), and the assumptions in the two theorems hold. Then, we have
\begin{align*}
    \mathrm{POE}(\HT) &\lesssim \sqrt{(\lambda_{k+1}^{\text{aug}}\rho_k(\SIG_{\text{aug}};n))^2 \cdot \left(\frac{n}{R_k(\SIG_{\text{aug}};n)} +\frac{k}{n}\right)\log n},\\
    \mathrm{MSE}(\HT) &\gtrsim (\lambda_{k+1}^{\text{aug}}\rho_k(\SIG_{\text{aug}};n))^2 +\left( \frac{n}{R_k(\SIG_{\text{aug}};n)} +\frac{k}{n}\right).
\end{align*}
As a consequence, the regression risk serves as a surrogate for the classification risk up to a $log$-factor:
\begin{align}
    \mathrm{POE}(\HT) \lesssim \mathrm{MSE}(\HT)\sqrt{\log n}.
\end{align}
\end{proposition}

To illustrate the implications of this proposition, let us consider the isotropic Gaussian noise injection augmentation with noise standard deviation $\sigma$ and random mask with dropout probability $\beta$ to train the 1-sparse model with a decaying data spectrum $\SIG_{ii}=\gamma^i,~\forall i\in\{1,2,\dots,p\}$, where $\gamma$ is some constant satisfying $0<\gamma<1$. Let $\hat{\T}_{\text{gn}}$ and $\hat{\T}_{\text{rm}}$ be the corresponding estimators. Then, a direct consequence of Proposition~\ref{gen_compare} (in conjunction with Corollaries~\ref{cor_rm},~\ref{rm-class},~\ref{gen_agn}, and~\ref{gn-class}) yields
\begin{align}\label{vv1}
    \lim_{n\rightarrow \infty}\lim_{\sigma\rightarrow \infty}\mathrm{POE}(\hat{\T}_{\text{gn}})= 0~~\text{while}~~\lim_{n\rightarrow \infty}\lim_{\sigma\rightarrow \infty}\mathrm{MSE}(\hat{\T}_{\text{gn}})= 1.
\end{align}
Also, when $p\log n\ll n$,
\begin{align}\label{vv2}
    \lim_{n\rightarrow \infty}\lim_{\beta\rightarrow 1}\mathrm{POE}(\hat{\T}_{\text{rm}})= 0~~\text{while}~~\lim_{n\rightarrow \infty}\lim_{\beta\rightarrow 1}\mathrm{MSE}(\hat{\T}_{\text{rm}})= 1.
\end{align}
\eqref{vv1} and \eqref{vv2} show that for both Gaussian noise injection and random mask augmentation, extreme augmentations can achieve perfect generalization in classification but poor generalization in regression.

It is worth noting that~\eqref{vv1} in particular studies an augmentation that significantly changes the data distribution.
In particular, for Gaussian injection augmentations we have
% Furthermore, we also want to remark that our framework is applicable to augmentation that significantly changes the data distribution. For example, the augmentation of Gaussian injection undergoes significant distributional shift, in the sense that
$
    \frac{W^2_2(g(\x),\x)}{p} \longrightarrow \infty \text{ as } n, \sigma \to \infty,
$
where $W_2$ denotes the 2-Wasserstein distance between the pre- and post-augmented distribution of the data by the Gaussian noise injection.
In Figs. \ref{fig:which_good}(b) and (d), we compare the Gaussian injection augmentation in the decaying spectrum $\gamma=0.95$ for regression and classification, respectively. We observe a
sharp difference between classification and regression,
where, as we increase the augmentation intensity (i.e.~variance of injected Gaussian noise), the MSE increases while the POE converges to a stable value (the ratio between SU and CN stays the same), implying that careful tuning is required for regression but not for classification. 
% Our last statement also shows that our framework can be used to analyze augmentation that has a strong distributional shift from the original distribution, complementing the analysis in \cite{chen2020group}, which assumes a small distributional shift. This message is coherent with the results of biased mask, see Section \ref{the ugly} and Fig. \ref{fig:bvub}, which we show has the same classification performance as unbiased mask while also inducing significant distributional shift.

Our second example that illustrates special benefits of DA in classification over regression concerns augmentations which are non-uniform across the features. In particular, if we allow different features to be augmented with different parameters, we can show that the induced spectrum $\SIG_{\text{aug}}$ can recover a ``bi-level'' design which was shown in Theorem 13 of \cite{muthukumar2020class} to separate classification and regression performance. We state this result for the case of non-uniform random mask in Appendix \ref{app:prop3}. It is worth noting that in the case where the true sparsity pattern is known, several augmentations (including non-uniform Gaussian noise injection, which incurs no approximation error in our analysis) can give rise to the same consistency behavior described above.

% The proof of the following proposition is deferred to Appendix \ref{app:prop3}.
% \end{remark}

% \begin{proposition}[\textbf{Non-uniform random mask is easier to tune in classification than regression}]\label{nurm_compare}
% Consider the 1-sparse model $\T^*=\sqrt{\frac{1}{\lambda_t}}\mathbf{e}_t$. Suppose the approximation error is not dominant in the bounds of Theorem \ref{gen_bound} (simple sufficient conditions can be found in Lemma \ref{cond_tight1}in Appendix \ref{appen:lemma}) and the assumptions in the two theorems hold. Suppose we apply the non-uniform random mask augmentation and recall the definitions of $\psi$ and $\psi_t$ as in Corollary \ref{hrm-class}. Then, if 
%     $\sqrt{\frac{p}{n}} \ll \frac{\psi}{\psi_t} \ll \frac{p}{n},$ we have 
% \begin{align}
%     \mathrm{POE}(\hat{\T}_{\text{rm}})\overset{n}{\longrightarrow} 0~~\text{while}~~\mathrm{MSE}(\hat{\T}_{\text{rm}})\overset{n}{\longrightarrow} 1.
% \end{align}
% \end{proposition}
% \begin{remark}
% By allowing the augmentation parameters $\psi$ and $\psi_1$ to vary with $n$, the induced spectrum $\SIG_{\text{aug}}$ recovers the ``bi-level'' design, which was shown in Theorem 13 of \cite{muthukumar2020class} to separate classification and regression performance. 
% It is worth noting that in the case where the true sparsity pattern is known, several augmentations (including nonuniform Gaussian noise injection, which incurs no approximation error in our analysis) can give rise to the same consistency behavior described above.
% \end{remark}
% \vidya{I realized that I had a technical question about the error bounds for the non-uniform augmentations: does the condition number in the independent-feature proposition grow with $n$? Is that dependence (for the approximation error) included in the bounds?}
% \henry{I suppose you mean the condition number $\kappa$ in our theorem? if so, it does not depend on $n$ but rather on the ratio between the largest and smallest dropout probability}
% \vidya{I was referring to Proposition 1 and the ratio $\sigma_i^2/\overline{\sigma}_i^2$. Does that remain constant even when dropout probabilities become very small or very large?}
% \henry{yes, i think so. because the ratio are defined within the same feature, so that wont be a problem, unless the quantity is like $\sigma_i/\sigma_j,i\neq j$. @chiraag can you help confirm my intuition is correct?
% }\chiraag{Yes, that's right - the mask probability will cancel since both quantities are for the same feature}

As a takeaway, the corollaries in this section demonstrate that the choice of augmentation itself can be more benign for classification tasks. Specifically, augmentations that are ``biased on average'' may perform similarly to their unbiased counterparts; we cannot generally expect this behavior for regression. Finally, we concluded this section by showing that our framework can be applied to strongly \emph{out-of-distribution} (OOD) augmentations, and show that strong distributional shift can sometimes lead to improvements in classification generalization. We observe the same phenomenon empirically in Fig. \ref{fig:which_good}, where increasing the intensity of the augmentation improves generalization and also increases the distributional shift.
